A Brief Study of In-Domain Transfer and Learning from Fewer Samples using A Few Simple Priors

Domain knowledge can often be encoded in the structure of a network, such as convolutional layers for vision, which has been shown to increase generalization and decrease sample complexity, or the number of samples required for successful learning. In this study, we ask whether sample complexity can be reduced for systems where the structure of the domain is unknown beforehand, and the structure and parameters must both be learned from the data. We show that sample complexity reduction through learning structure is possible for at least two simple cases. In studying these cases, we also gain insight into how this might be done for more complex domains.

==> marcbib <==
@article{kirkpatrick2017overcoming,
  title={Overcoming catastrophic forgetting in neural networks},
  author={Kirkpatrick, James and Pascanu, Razvan and Rabinowitz, Neil and Veness, Joel and Desjardins, Guillaume and Rusu, Andrei A and Milan, Kieran and Quan, John and Ramalho, Tiago and Grabska-Barwinska, Agnieszka and others},
  journal={Proceedings of the National Academy of Sciences},
  pages={201611835},
  year={2017},
  publisher={National Acad Sciences}
}

@article{pickett2016growing,
  title={A Growing Long-term Episodic \& Semantic Memory},
  author={Pickett, Marc and Al-Rfou, Rami and Shao, Louis and Tar, Chris},
  journal={arXiv preprint arXiv:1610.06402},
  year={2016}
}

@inproceedings{andrychowicz2016learning,
  title={Learning to learn by gradient descent by gradient descent},
  author={Andrychowicz, Marcin and Denil, Misha and Gomez, Sergio and Hoffman, Matthew W and Pfau, David and Schaul, Tom and de Freitas, Nando},
  booktitle={Advances in Neural Information Processing Systems},
  pages={3981--3989},
  year={2016}
}

@book{thrun2012learning,
  title={Learning to learn},
  author={Thrun, Sebastian and Pratt, Lorien},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{luong2015multi,
  title={Multi-task sequence to sequence learning},
  author={Luong, Minh-Thang and Le, Quoc V and Sutskever, Ilya and Vinyals, Oriol and Kaiser, Lukasz},
  journal={arXiv preprint arXiv:1511.06114},
  year={2015}
}

@phdthesis{ring:1994,
  AUTHOR    = {M. Ring},
  TITLE     = {{Continual Learning in Reinforcement Environments}},
  SCHOOL    = {{University of Texas at Austin}},
  YEAR      = {1994},
  type      = {Doctoral dissertation},
}


@article{ruvolo2013ella,
  title={ELLA: An Efficient Lifelong Learning Algorithm.},
  author={Ruvolo, Paul and Eaton, Eric},
  journal={ICML (1)},
  volume={28},
  pages={507--515},
  year={2013}
}

@techreport{taylor2016lifelong,
  title={Lifelong Transfer Learning for Heterogeneous Teams of Agents in Sequential Decision Processes},
  author={Taylor, Matthew and Eaton, Eric and Ruvolo, Paul},
  year={2016},
  institution={Washington State University Pullman United States}
}

@article{pan2010survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2010},
  publisher={IEEE}
}

@article{zhou2016latent,
  title={Latent Contextual Bandits and their Application to Personalized Recommendations for New Users},
  author={Zhou, Li and Brunskill, Emma},
  journal={arXiv preprint arXiv:1604.06743},
  year={2016}
}

@article{dudik2011efficient,
  title={Efficient optimal learning for contextual bandits},
  author={Dudik, Miroslav and Hsu, Daniel and Kale, Satyen and Karampatziakis, Nikos and Langford, John and Reyzin, Lev and Zhang, Tong},
  journal={arXiv preprint arXiv:1106.2369},
  year={2011}
}

@article{blei2003latent,
  title={Latent dirichlet allocation},
  author={Blei, David M and Ng, Andrew Y and Jordan, Michael I},
  journal={Journal of machine Learning research},
  volume={3},
  number={Jan},
  pages={993--1022},
  year={2003}
}

@article{wolpert1997no,
  title={No free lunch theorems for optimization},
  author={Wolpert, David H and Macready, William G},
  journal={IEEE transactions on evolutionary computation},
  volume={1},
  number={1},
  pages={67--82},
  year={1997},
  publisher={IEEE}
}

@inproceedings{sutskever2014sequence,
  title={Sequence to sequence learning with neural networks},
  author={Sutskever, Ilya and Vinyals, Oriol and Le, Quoc V},
  booktitle={Advances in neural information processing systems},
  pages={3104--3112},
  year={2014}
}

@article{blundell2016model,
  title={Model-free episodic control},
  author={Blundell, Charles and Uria, Benigno and Pritzel, Alexander and Li, Yazhe and Ruderman, Avraham and Leibo, Joel Z and Rae, Jack and Wierstra, Daan and Hassabis, Demis},
  journal={arXiv preprint arXiv:1606.04460},
  year={2016}
}

@article{oh2016control,
  title={Control of Memory, Active Perception, and Action in Minecraft},
  author={Oh, Junhyuk and Chockalingam, Valliappa and Singh, Satinder and Lee, Honglak},
  journal={arXiv preprint arXiv:1605.09128},
  year={2016}
}

@article{graves2014neural,
  title={Neural turing machines},
  author={Graves, Alex and Wayne, Greg and Danihelka, Ivo},
  journal={arXiv preprint arXiv:1410.5401},
  year={2014}
}

@article{weston2014memory,
  title={Memory networks},
  author={Weston, Jason and Chopra, Sumit and Bordes, Antoine},
  journal={arXiv preprint arXiv:1410.3916},
  year={2014}
}

@inproceedings{reisinger2004evolving,
  title={Evolving reusable neural modules},
  author={Reisinger, Joseph and Stanley, Kenneth O and Miikkulainen, Risto},
  booktitle={Genetic and Evolutionary Computation Conference},
  pages={69--81},
  year={2004},
  organization={Springer}
}

@inproceedings{li2016learning,
  title={Learning without Forgetting},
  author={Li, Zhizhong and Hoiem, Derek},
  booktitle={European Conference on Computer Vision},
  pages={614--629},
  year={2016},
  organization={Springer}
}

@book{hollander2013nonparametric,
  title={Nonparametric statistical methods},
  author={Hollander, Myles and Wolfe, Douglas A and Chicken, Eric},
  year={2013},
  publisher={John Wiley \& Sons}
}

@article{fritzke1995growing,
  title={A growing neural gas network learns topologies},
  author={Fritzke, Bernd and others},
  journal={Advances in neural information processing systems},
  volume={7},
  pages={625--632},
  year={1995},
  publisher={Citeseer}
}

@article{fahlman1989cascade,
  title={The cascade-correlation learning architecture},
  author={Fahlman, Scott E and Lebiere, Christian},
  year={1989}
}

@article{chen2015net2net,
  title={Net2net: Accelerating learning via knowledge transfer},
  author={Chen, Tianqi and Goodfellow, Ian and Shlens, Jonathon},
  journal={arXiv preprint arXiv:1511.05641},
  year={2015}
}

@article{cortes2016adanet,
  title={AdaNet: Adaptive Structural Learning of Artificial Neural Networks},
  author={Cortes, Corinna and Gonzalvo, Xavi and Kuznetsov, Vitaly and Mohri, Mehryar and Yang, Scott},
  journal={arXiv preprint arXiv:1607.01097},
  year={2016}
}

@article{reed2015neural,
  title={Neural programmer-interpreters},
  author={Reed, Scott and de Freitas, Nando},
  journal={arXiv preprint arXiv:1511.06279},
  year={2015}
}

@article{rusu2016progressive,
  title={Progressive Neural Networks},
  author={Rusu, Andrei A and Rabinowitz, Neil C and Desjardins, Guillaume and Soyer, Hubert and Kirkpatrick, James and Kavukcuoglu, Koray and Pascanu, Razvan and Hadsell, Raia},
  journal={arXiv preprint arXiv:1606.04671},
  year={2016}
}

@misc{openaigym,
        Author = {Greg Brockman and Vicki Cheung and Ludwig Pettersson and Jonas Schneider and John Schulman and Jie Tang and Wojciech Zaremba},
        Title = {OpenAI Gym},
        Year = {2016},
        Eprint = {arXiv:1606.01540},
}

@article{wang2014hashing,
  title={Hashing for similarity search: A survey},
  author={Wang, Jingdong and Shen, Heng Tao and Song, Jingkuan and Ji, Jianqiu},
  journal={arXiv preprint arXiv:1408.2927},
  year={2014}
}

@inproceedings{gionis1999similarity,
  title={Similarity search in high dimensions via hashing},
  author={Gionis, Aristides and Indyk, Piotr and Motwani, Rajeev and others},
  booktitle={VLDB},
  volume={99},
  number={6},
  pages={518--529},
  year={1999}
}

@article{stewart2011biologically,
  title={A biologically realistic cleanup memory: Autoassociation in spiking neurons},
  author={Stewart, Terrence C and Tang, Yichuan and Eliasmith, Chris},
  journal={Cognitive Systems Research},
  volume={12},
  number={2},
  pages={84--92},
  year={2011},
  publisher={Elsevier}
}

@article{bartol2015nanoconnectomic,
  title={Nanoconnectomic upper bound on the variability of synaptic plasticity},
  author={Bartol Jr, Thomas M and Bromer, Cailey and Kinney, Justin and Chirillo, Michael A and Bourne, Jennifer N and Harris, Kristen M and Sejnowski, Terrence J},
  journal={Elife},
  volume={4},
  pages={e10778},
  year={2015},
  publisher={eLife Sciences Publications Limited}
}

@article{he2015deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  journal={arXiv preprint arXiv:1512.03385},
  year={2015}
}

@article{drachman2005we,
  title={Do we have brain to spare?},
  author={Drachman, David A},
  journal={Neurology},
  volume={64},
  number={12},
  pages={2004--2005},
  year={2005},
  publisher={AAN Enterprises}
}

@inproceedings{trask2015modeling,
  title={Modeling order in neural word embeddings at scale},
  author={Trask, Andrew and Gilmore, David and Russell, Matthew},
  booktitle={Proceedings of the 32nd International Conference on Machine Learning (ICML)},
  pages={2266--2275},
  year={2015}
}

@article{pakkenberg1997neocortical,
  title={Neocortical neuron number in humans: effect of sex and age},
  author={Pakkenberg, Bente and Gundersen, Hans J{\o}rgen G},
  journal={Journal of Comparative Neurology},
  volume={384},
  number={2},
  pages={312--320},
  year={1997},
  publisher={Wiley Online Library}
}

@article{nguyen2010total,
  title={Total number of synapses in the adult human neocortex},
  author={Nguyen, Thai},
  journal={Undergraduate Journal of Mathematical Modeling: One+ Two},
  volume={3},
  number={1},
  pages={26},
  year={2010}
}

@article{azevedo2009equal,
  title={Equal numbers of neuronal and nonneuronal cells make the human brain an isometrically scaled-up primate brain},
  author={Azevedo, Frederico AC and Carvalho, Ludmila RB and Grinberg, Lea T and Farfel, Jos{\'e} Marcelo and Ferretti, Renata EL and Leite, Renata EP and Lent, Roberto and Herculano-Houzel, Suzana and others},
  journal={Journal of Comparative Neurology},
  volume={513},
  number={5},
  pages={532--541},
  year={2009},
  publisher={Wiley Online Library}
}

@inproceedings{silver2013lifelong,
  title={Lifelong Machine Learning Systems: Beyond Learning Algorithms.},
  author={Silver, Daniel L and Yang, Qiang and Li, Lianghao},
  booktitle={AAAI Spring Symposium: Lifelong Machine Learning},
  pages={49--55},
  year={2013}
}

@article{aha1991instance,
  title={Instance-based learning algorithms},
  author={Aha, David W and Kibler, Dennis and Albert, Marc K},
  journal={Machine learning},
  volume={6},
  number={1},
  pages={37--66},
  year={1991},
  publisher={Kluwer Academic Publishers}
}

@article{dere2006case,
  title={The case for episodic memory in animals},
  author={Dere, E and Kart-Teke, E and Huston, JP and Silva, MA De Souza},
  journal={Neuroscience \& Biobehavioral Reviews},
  volume={30},
  number={8},
  pages={1206--1224},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{ammar2015autonomous,
  title={Autonomous cross-domain knowledge transfer in lifelong policy gradient reinforcement learning},
  author={Ammar, Haitham Bou and Eaton, Eric and Luna, Jos{\'e} Marcio and Ruvolo, Paul},
  booktitle={Proc. of IJCAI},
  year={2015}
}

@article{kumar2015ask,
  title={Ask me anything: Dynamic memory networks for natural language processing},
  author={Kumar, Ankit and Irsoy, Ozan and Su, Jonathan and Bradbury, James and English, Robert and Pierce, Brian and Ondruska, Peter and Gulrajani, Ishaan and Socher, Richard},
  journal={arXiv preprint arXiv:1506.07285},
  year={2015}
}

@BOOK{Thrun96b,
  AUTHOR         = {S. Thrun},
  YEAR           = {1996},
  TITLE          = {Explanation-Based Neural Network Learning: A Lifelong Learning Approach},
  PUBLISHER      = {Kluwer Academic Publishers},
  ADDRESS        = {Boston, MA}
}

@book{heinlein,
  author={Robert A. Heinlein},
  year={1973},
  title={Time Enough for Love},
  publisher={G.P. Putnam's Sons},
  address={New York, NY},
  isbn={0-399-11151-4}
}

@article{mnih2015human,
  title={Human-level control through deep reinforcement learning},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
  journal={Nature},
  volume={518},
  number={7540},
  pages={529--533},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{schmidhuber2015learning,
  title={On Learning to Think: Algorithmic Information Theory for Novel Combinations of Reinforcement Learning Controllers and Recurrent Neural World Models},
  author={Schmidhuber, Juergen},
  journal={arXiv preprint arXiv:1511.09249},
  year={2015}
}

@article{lake2016building,
  title={Building Machines That Learn and Think Like People},
  author={Lake, Brenden M and Ullman, Tomer D and Tenenbaum, Joshua B and Gershman, Samuel J},
  journal={arXiv preprint arXiv:1604.00289},
  year={2016}
}

@article{o2014complementary,
  title={Complementary learning systems},
  author={O’Reilly, Randall C and Bhattacharyya, Rajan and Howard, Michael D and Ketz, Nicholas},
  journal={Cognitive Science},
  volume={38},
  number={6},
  pages={1229--1248},
  year={2014},
  publisher={Wiley Online Library}
}

@article{yartsev2013representation,
  title={Representation of three-dimensional space in the hippocampus of flying bats},
  author={Yartsev, Michael M and Ulanovsky, Nachum},
  journal={Science},
  volume={340},
  number={6130},
  pages={367--372},
  year={2013},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{bakker2001reinforcement,
  title={Reinforcement Learning with Long Short-Term Memory.},
  author={Bakker, Bram},
  booktitle={NIPS},
  pages={1475--1482},
  year={2001}
}

@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

@article{fisher1985narrative,
  title={The narrative paradigm: An elaboration},
  author={Fisher, Walter R},
  journal={Communications Monographs},
  volume={52},
  number={4},
  pages={347--367},
  year={1985},
  publisher={Taylor \& Francis}
}

@book{kurzweil2012create,
  title={How to create a mind: The secret of human thought revealed},
  author={Kurzweil, Ray},
  year={2012},
  publisher={Penguin}
}

@inproceedings{sutskever2009recurrent,
  title={The recurrent temporal restricted boltzmann machine},
  author={Sutskever, Ilya and Hinton, Geoffrey E and Taylor, Graham W},
  booktitle={Advances in Neural Information Processing Systems},
  pages={1601--1608},
  year={2009}
}

@article{fine1998hierarchical,
  title={The hierarchical hidden Markov model: Analysis and applications},
  author={Fine, Shai and Singer, Yoram and Tishby, Naftali},
  journal={Machine learning},
  volume={32},
  number={1},
  pages={41--62},
  year={1998},
  publisher={Springer}
}

@article{moser2008place,
  title={Place cells, grid cells, and the brain's spatial representation system},
  author={Moser, Edvard I and Kropff, Emilio and Moser, May-Britt},
  journal={Annu. Rev. Neurosci.},
  volume={31},
  pages={69--89},
  year={2008},
  publisher={Annual Reviews}
}

@article{tolman1948cognitive,
  title={Cognitive maps in rats and men.},
  author={Tolman, Edward C},
  journal={Psychological review},
  volume={55},
  number={4},
  pages={189},
  year={1948},
  publisher={American Psychological Association}
}

@article{buzsaki2013memory,
  title={Memory, navigation and theta rhythm in the hippocampal-entorhinal system},
  author={Buzs{\'a}ki, Gy{\"o}rgy and Moser, Edvard I},
  journal={Nature neuroscience},
  volume={16},
  number={2},
  pages={130--138},
  year={2013},
  publisher={Nature Publishing Group}
}

@book{hofstadter2013surfaces,
  title={Surfaces and Essences: Analogy as the Fuel and Fire of Thinking},
  author={Hofstadter, Douglas and Sander, Emmanuel},
  year={2013},
  publisher={Basic Books}
}

@inproceedings{dean2012three,
  title={Three Controversial Hypotheses Concerning Computation in the Primate Cortex.},
  author={Dean, Thomas L and Corrado, Greg and Shlens, Jonathon},
  booktitle={AAAI},
  year={2012}
}

@article{Battaglia05112013,
author = {Battaglia, Peter W. and Hamrick, Jessica B. and Tenenbaum, Joshua B.},
title = {Simulation as an engine of physical scene understanding},
volume = {110},
number = {45},
pages = {18327-18332},
year = {2013},
doi = {10.1073/pnas.1306572110},
abstract ={In a glance, we can perceive whether a stack of dishes will topple, a branch will support a child’s weight, a grocery bag is poorly packed and liable to tear or crush its contents, or a tool is firmly attached to a table or free to be lifted. Such rapid physical inferences are central to how people interact with the world and with each other, yet their computational underpinnings are poorly understood. We propose a model based on an “intuitive physics engine,” a cognitive mechanism similar to computer engines that simulate rich physics in video games and graphics, but that uses approximate, probabilistic simulations to make robust and fast inferences in complex natural scenes where crucial information is unobserved. This single model fits data from five distinct psychophysical tasks, captures several illusions and biases, and explains core aspects of human mental models and common-sense reasoning that are instrumental to how humans understand their everyday world.},
URL = {http://www.pnas.org/content/110/45/18327.abstract},
eprint = {http://www.pnas.org/content/110/45/18327.full.pdf+html},
journal = {Proceedings of the National Academy of Sciences}
}

@inproceedings{pickett:2013b,
  author = {Pickett, M.},
  booktitle = {Advances in Cognitive Systems Workshop on Metacognition about Artificial Situated Agents},
  title = {{Towards A Unified Framework for Learning and Processing Perceptual, Relational, and Meta Knowledge}},
  year = {2013}
}

@inproceedings{heitmeyer+pickett+al:2013,
  author = {Heitmeyer, C. and Pickett, M. and Breslow, L. and Aha, D.W. and Trafton, J.G. and Leonard, E.I.},
  booktitle = {Proceedings of the 2nd International NSF sponsored Workshop on Realizing Artificial Intelligence Synergies in Software Engineering (RAISE'13)},
  title = {{High Assurance Human-Centric Decision Systems}},
  year = {2013}
}

@inproceedings{pickett:2013,
  author = {Pickett, M.},
  booktitle = {AAAI Workshop on Learning Rich Representations from Low-Level Sensors},
  title = {{Building on Deep Learning}},
  year = {2013}
}

@article{cox2005metacognition,
  title={Metacognition in computation: A selected research review},
  author={Cox, Michael T},
  journal={Artificial Intelligence},
  volume={169},
  number={2},
  pages={104--141},
  year={2005},
  publisher={Elsevier}
}

@article{smith2009study,
  title={The study of animal metacognition},
  author={Smith, J David},
  journal={Trends in cognitive sciences},
  volume={13},
  number={9},
  pages={389--396},
  year={2009},
  publisher={Elsevier}
}

@article{carruthers2008meta,
  title={Meta-cognition in animals: A skeptical look},
  author={Carruthers, Peter},
  journal={Mind \& Language},
  volume={23},
  number={1},
  pages={58--89},
  year={2008},
  publisher={Wiley Online Library}
}

@article{Pickett2013,
title = "Using cortically-inspired algorithms for analogical learning and reasoning ",
journal = "Biologically Inspired Cognitive Architectures ",
volume = "6",
year = "2013",
pages="76-86",
issn = "2212-683X",
doi = "http://dx.doi.org/10.1016/j.bica.2013.07.003",
url = "http://www.sciencedirect.com/science/article/pii/S2212683X13000704",
author = "Marc Pickett and David W. Aha",
}

@article{granger2011brains,
  title={How Brains Are Built: Principles of Computational Neuroscience},
  author={Granger, Richard},
  journal={Cerebrum; The Dana Foundation},
  year={2011}
}

@article{chandrashekar2011derivation,
  title={Derivation of a novel efficient supervised learning algorithm from cortical-subcortical loops},
  author={Chandrashekar, Ashok and Granger, Richard},
  journal={Frontiers in computational neuroscience},
  volume={5},
  year={2011},
  publisher={Frontiers Media SA}
}

@article{granger2006engines,
  title={Engines of the brain: The computational instruction set of human cognition},
  author={Granger, Richard},
  journal={AI Magazine},
  volume={27},
  number={2},
  pages={15},
  year={2006}
}

@article{yaner2006visual,
  title={Visual analogy: Viewing analogical retrieval and mapping as constraint satisfaction problems},
  author={Yaner, Patrick W and Goel, Ashok K},
  journal={Applied Intelligence},
  volume={25},
  number={1},
  pages={91--105},
  year={2006},
  publisher={Springer}
}

@article{rilling2006human,
  title={{Human and Nonhuman Primate Brains: Are they Allometrically Scaled Versions of the Same Design?}},
  author={Rilling, James K},
  journal={Evolutionary Anthropology: Issues, News, and Reviews},
  volume={15},
  number={2},
  pages={65--77},
  year={2006},
  publisher={Wiley Online Library}
}

@article{deacon1997makes,
  title={{What Makes the Human Brain Different?}},
  author={Deacon, Terrence W},
  journal={Annual Review of Anthropology},
  pages={337--357},
  year={1997},
  publisher={JSTOR}
}

@article{marcus1998rethinking,
  title={Rethinking eliminative connectionism},
  author={Marcus, Gary F},
  journal={Cognitive Psychology},
  volume={37},
  number={3},
  pages={243--282},
  year={1998},
  publisher={Elsevier}
}

@article{sur2005patterning,
  title={Patterning and plasticity of the cerebral cortex},
  author={Sur, Mriganka and Rubenstein, John LR},
  journal={Science Signaling},
  volume={310},
  number={5749},
  pages={805},
  year={2005},
  publisher={AAAS}
}

@inproceedings{pickett+aha:2013,
  title={{Spontaneous Analogy by Piggybacking on a Perceptual System}},
  author={Pickett, M. and Aha, D.W.},
  booktitle={{Proceedings of the 35th Annual Conference of the Cognitive Science Society}},
  editor = {Knauff, M and Pauen, M and Sebanz, N and Wachsmuth, I},
  address = {Austin, TX},
  pages={3229-3234},
  year={2013}
}

@article{rachkovskij2012building,
  title={{Building a World Model with Structure-Sensitive Sparse Binary Distributed Representations}},
  author={Rachkovskij, D.A. and Kussul, E.M. and Baidyk, T.N.},
  journal={Bio. Inspired Cog. Archs.},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{pickett+aha+trafton:2013,
  Author = {Marc Pickett and David W. Aha and J. Gregory Trafton},
  Title = {Acquiring User Models to test automated assistants},
  Year = {2013},
  booktitle={Proceedings of the Twenty-Sixth International Florida Artificial Intelligence Research Society Conference},
  organization={AAAI Press}
}

@inproceedings{quoc:2012,
title = {{Building High-Level Features using Large Scale Unsupervised Learning}},
author  = {Quoc Le and Marc'Aurelio Ranzato and Rajat Monga and Matthieu Devin and Kai Chen and Greg Corrado and Jeff Dean and Andrew Ng},
year  = 2012,
booktitle = {International Conference in Machine Learning}
}

@article{anderson2010neural,
  title={Neural reuse: A fundamental organizational principle of the brain},
  author={Anderson, M.L.},
  journal={Behavioral and Brain Sciences},
  volume={33},
  number={4},
  pages={245--266},
  year={2010},
  publisher={Cambridge Univ Press}
}

@inproceedings{Kuehne00seql:category,
  title={{SEQL: Category Learning as Progressive Abstraction Using Structure Mapping}},
  author={Kuehne, S. and Forbus, K. and Gentner, D. and Quinn, B.},
  booktitle={{Proceedings of the 22nd Annual Meeting of the Cognitive Science Society}},
  year={2000},
  address={}
}

@inproceedings{DBLP:conf/context/KokinovG01,
  author    = {Boicho N. Kokinov and  Maurice Grinberg},
  title     = {{Simulating Context Effects in Problem Solving with AMBR}},
  booktitle = {CONTEXT},
  year      = {2001},
  pages     = {221-234},
  ee        = {http://dx.doi.org/10.1007/3-540-44607-9_17},
  crossref  = {DBLP:conf/context/2001},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/context/2001,
  editor    = {Varol Akman and
               Paolo Bouquet and
               Richmond H. Thomason and
               Roger A. Young},
  title     = {{Modeling and Using Context, Third International and Interdisciplinary
               Conference, CONTEXT, 2001, Dundee, UK, July 27-30, 2001,
               Proceedings}},
  booktitle = {CONTEXT},
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {2116},
  year      = {2001},
  isbn      = {3-540-42379-6},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{DBLP:journals/ai/Smolensky90,
  author    = {Paul Smolensky},
  title     = {{Tensor Product Variable Binding and the Representation of
               Symbolic Structures in Connectionist Systems}},
  journal   = {Artif. Intell.},
  volume    = {46},
  number    = {1-2},
  year      = {1990},
  pages     = {159-216},
  ee        = {http://dx.doi.org/10.1016/0004-3702(90)90007-M},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{hummel+holyoak+green+doumas:2004,
  title={{A Solution to the Binding Problem for Compositional Connectionism}},
  author={Hummel, J. E. and Holyoak, K. J. and Green, C. and Doumas, L. A. A. and Devnich, D. and Kittur, A. and  Kalar, D. J.},
  booktitle={{AAAI Fall Symp. on Comp. Connectionism in Cog. Sci}},
  year={2004},
  address={}
}

@book{jackendoff02,
  author={Ray Jackendoff},
  title={{Foundations of Language: Brain, Meaning, Grammar, Evolution}},
  year={2002},
  publisher={Oxford University Press},
  url={http://www.isrl.uiuc.edu/~amag/langev/paper/jackendoff02.html}
}

@inproceedings{mclure+friedman+forbus:2010,
  title={{Learning Concepts from Sketches via Analogical Generalization and Near-misses}},
  author={McLure, M. and Friedman, S. E. and Forbus, K. D.},
  booktitle={{Proceedings of the 32nd Annual Conference of the Cognitive Science Society. Portland, OR.}},
  year={2010}
}

@article{klenk+forbus:2009,
  title={{Domain Transfer via Cross-Domain Analogy}},
  author={Klenk, M. and Forbus, K. D.},
  journal={Cognitive Systems Research, Special Issue on Analogies: Integrating Cognitive Abilities.},
  publisher = {Elsevier},
  year={2009}
}


@inproceedings{kanerva2010we,
  title={{What We Mean When We Say ``What's the Dollar of Mexico?'': Prototypes and Mapping in Concept Space}},
  author={Kanerva, P.},
  booktitle={2010 AAAI Fall Symposium Series},
  year={2010}
}

@article{citeulike:3033318,
    abstract = {{Human cognition is unique in the way in which it relies on combinatorial (or compositional) structures. Language provides ample evidence for the existence of combinatorial structures, but they can also be found in visual cognition. To understand the neural basis of human cognition, it is therefore essential to understand how combinatorial structures can be instantiated in neural terms. In his recent book on the foundations of language, Jackendoff described four fundamental problems for a neural instantiation of combinatorial structures: the massiveness of the binding problem, the problem of 2, the problem of variables, and the transformation of combinatorial structures from working memory to long-term memory. This paper aims to show that these problems can be solved by means of neural \&ldquo;blackboard\&rdquo; architectures. For this purpose, a neural blackboard architecture for sentence structure is presented. In this architecture, neural structures that encode for words are temporarily bound in a manner that preserves the structure of the sentence. It is shown that the architecture solves the four problems presented by Jackendoff. The ability of the architecture to instantiate sentence structures is illustrated with examples of sentence complexity observed in human language performance. Similarities exist between the architecture for sentence structure and blackboard architectures for combinatorial structures in visual cognition, derived from the structure of the visual cortex. These architectures are briefly discussed, together with an example of a combinatorial structure in which the blackboard architectures for language and vision are combined. In this way, the architecture for language is grounded in perception. Perspectives and potential developments of the architectures are discussed.}},
    author = {van der Velde, Frank and de Kamps, Marc},
    citeulike-article-id = {3033318},
    citeulike-linkout-0 = {http://journals.cambridge.org/action/displayAbstract?fromPage=online\&aid=414583},
    citeulike-linkout-1 = {http://dx.doi.org/10.1017/S0140525X06009022},
    day = {15},
    doi = {10.1017/S0140525X06009022},
    journal = {Behavioral and Brain Sciences},
    keywords = {binding, combinatorial, language, problem},
    number = {01},
    pages = {37--70},
    posted-at = {2008-07-22 18:51:52},
    priority = {2},
    title = {{Neural Blackboard Architectures of Combinatorial Structures in Cognition}},
    volume = {29},
    year = {2006}
}

@inproceedings{FloydE10-ICCBRGames,
  author = {Michael W. Floyd and Babak Esfandiari},
  booktitle = {Workshop on Case-Based Reasoning for Computer Games at the 18th International Conference on Case-Based Reasoning, ICCBR 2010, Alessandria, Italy, July 19-22, 2010. Proceedings},
  title = {{Toward a Domain-independent Case-based Reasoning Approach for Imitation: Three Case Studies in Gaming}},
  year = {2010},
  pages = {55-64}
}

@INPROCEEDINGS{Galata99learningbehaviour,
    author = {Aphrodite Galata and Neil Johnson and David Hogg},
    title = {{Learning Behaviour Models of Human Activities}},
    booktitle = {In Proc. BMVC},
    year = {1999},
    pages = {12--22}
}

@article{Argall:2009:SRL:1523530.1524008,
 author = {Argall, Brenna D. and Chernova, Sonia and Veloso, Manuela and Browning, Brett},
 title = {A survey of robot learning from demonstration},
 journal = {Robot. Auton. Syst.},
 volume = {57},
 issue = {5},
 month = {May},
 year = {2009},
 issn = {0921-8890},
 pages = {469--483},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=1523530.1524008},
 doi = {10.1016/j.robot.2008.10.024},
 acmid = {1524008},
 publisher = {North-Holland Publishing Co.},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {Autonomous systems, Learning from demonstration, Machine learning, Robotics},
}

@inproceedings{DBLP:conf/icml/SammutHKM92,
  author    = {Claude Sammut and
               Scott Hurst and
               Dana Kedzier and
               Donald Michie},
  title     = {Learning to Fly},
  booktitle = {ML},
  year      = {1992},
  pages     = {385-393},
  crossref  = {DBLP:conf/icml/1992},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/icml/1992,
  editor    = {Derek H. Sleeman and
               Peter Edwards},
  title     = {Proceedings of the Ninth International Workshop on Machine
               Learning (ML 1992), Aberdeen, Scotland, UK, July 1-3, 1992},
  booktitle = {ML},
  publisher = {Morgan Kaufmann},
  year      = {1992},
  isbn      = {1-55860-247-X},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DBLP:conf/icml/IsaacS03,
  author    = {Andrew Isaac and
               Claude Sammut},
  title     = {Goal-directed Learning to Fly},
  booktitle = {ICML},
  year      = {2003},
  pages     = {258-265},
  crossref  = {DBLP:conf/icml/2003},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/icml/2003,
  editor    = {Tom Fawcett and
               Nina Mishra},
  title     = {Machine Learning, Proceedings of the Twentieth International
               Conference (ICML 2003), August 21-24, 2003, Washington,
               DC, USA},
  publisher = {AAAI Press},
  year      = {2003},
  isbn      = {1-57735-189-4},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DBLP:conf/mi/BainS95,
  author    = {Michael Bain and
               Claude Sammut},
  title     = {A Framework for Behavioural Cloning},
  booktitle = {Machine Intelligence 15},
  year      = {1995},
  pages     = {103-129},
  crossref  = {DBLP:conf/mi/1995},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/mi/1995,
  editor    = {Koichi Furukawa and
               Donald Michie and
               Stephen Muggleton},
  title     = {Machine Intelligence 15, Intelligent Agents [St. Catherine's
               College, Oxford, July 1995]},
  booktitle = {Machine Intelligence 15},
  publisher = {Oxford University Press},
  year      = {1999},
  isbn      = {0-19-853867-7},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@InProceedings{baldwin+goldstone:2007,
  AUTHOR    = {D. Baldwin and R. L. Goldstone},
  TITLE     = {{Finding Analogies Within Systems: Constraints on Unsegmented Matching}},
  BOOKTITLE = {{WrkShp. on Analogies: Integrating Multiple Cog. Abilities}},
  YEAR      = {2007},
  ADDRESS   = {}
}

@article{pollack1990recursive,
  title={Recursive distributed representations},
  author={Pollack, J.B.},
  journal={Artificial Intelligence},
  volume={46},
  number={1-2},
  pages={77--105},
  year={1990},
  publisher={Elsevier}
}

@inproceedings{forbus2008companion,
  title={{Companion cognitive systems: Design goals and some lessons learned}},
  author={Forbus, K. and Klenk, M. and Hinrichs, T.},
  booktitle={AAAI Fall Symposium on Naturally Inspired Artificial Intelligence},
  year={2008}
}

@article{french2000coffee,
  title={{When Coffee Cups are Like Old Elephants, or Why Representation Modules Don't Make Sense}},
  author={French, R.},
  journal={Understanding Representation in the Cognitive Sciences},
  pages={93--100},
  year={2000},
  publisher={Springer}
}

@phdthesis{morrison1998situated,
  title={Situated representation: Solving the handcoding problem with emergent structured representation},
  author={Morrison, C.T.},
  year={1998},
  school={State University of New York}
}

@phdthesis{nehme:2009,
  title={Modeling Human Supervisory Control in Heterogeneous Unmanned Vehicle System},
  author={Nehme, C.E.},
  year={2009},
  school={MIT Dept. of Aeronautics and Astronautics, Cambridge, MA.}
}

@inproceedings{socher2012semantic,
  title={{Semantic Compositionality through Recursive Matrix-Vector Spaces}},
  author={Socher, R. and Huval, B. and Manning, C. D. and Ng, A. Y.},
  booktitle={Proceedings of the Joint Conference on Empirical Methods in Natural Language Processing and Computational Natural Language Learning},
  year={2012},
}

@inproceedings{socher2011parsing,
  title={Parsing Natural Scenes and Natural Language with Recursive Neural Networks},
  author={Socher, R. and Lin, C.C.Y. and Ng, A.Y. and Manning, C.D.},
  booktitle    = "Proceedings of International Conference on Machine Learning (ICML)",
  year={2011},
  organization={ICML}
}

@article{barsalou1999perceptual,
  title={Perceptual symbol systems},
  author={Barsalou, L.W.},
  journal={Behavioral and brain sciences},
  volume={22},
  number={04},
  pages={577--660},
  year={1999},
  publisher={Cambridge Univ Press}
}

@article{bar2006top,
  title={Top-down facilitation of visual recognition},
  author={Bar, M. and Kassam, K.S. and Ghuman, A.S. and Boshyan, J. and Schmid, A.M. and Dale, A.M. and H{\"a}m{\"a}l{\"a}inen, MS and Marinkovic, K. and Schacter, DL and Rosen, BR and others},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={103},
  number={2},
  pages={449},
  year={2006},
  publisher={National Acad Sciences}
}

@article{engel2001dynamic,
  title={Dynamic predictions: oscillations and synchrony in top-down processing},
  author={Engel, A.K. and Fries, P. and Singer, W.},
  journal={Nature Reviews Neuroscience},
  volume={2},
  number={10},
  pages={704--716},
  year={2001}
}

@article{falkenhainer1990unified,
  title={A unified approach to explanation and theory formation},
  author={Falkenhainer, B.},
  journal={Readings in Machine Learning},
  pages={373--403},
  year={1990}
}

@inproceedings{forbus2008cogsketch,
  title={{CogSketch: Open-domain sketch understanding for cognitive science research and for education}},
  author={Forbus, K. and Usher, J. and Lovett, A. and Lockwood, K. and Wetzel, J.},
  booktitle={Proceedings of the fifth eurographics workshop on sketch-based interfaces and modeling},
  year={2008}
}

@article{thagard1990analog,
  title={{Analog Retrieval by Constraint Satisfaction}},
  author={Thagard, P. and Holyoak, K.J. and Nelson, G. and Gochfeld, D.},
  journal={Artificial Intelligence},
  volume={46},
  number={3},
  pages={259--310},
  year={1990},
  publisher={Elsevier}
}

@article{forbus1995mac,
  title={{MAC/FAC: A Model of Similarity-based Retrieval}},
  author={Forbus, K.D. and Gentner, D. and Law, K.},
  journal={Cog. Sci.},
  volume={19},
  number={2},
  year={1995},
  publisher={Elsevier}
}

@book{mitchell1993analogy,
  title={{Analogy-Making as Perception: A Computer Model}},
  author={Mitchell, M.},
  publisher = {MIT Press},
  address = {Cambridge, MA, USA},
  year={1993}
}

@article{DBLP:journals/jetai/ChalmersFH92,
  author    = {David J. Chalmers and
               Robert M. French and
               Douglas Hofstadter},
  title     = {{High-level Perception, Representation, and Analogy: A Critique
               of Artificial Intelligence Methodology}},
  journal   = {J. Exp. Theor. Artif. Intell.},
  volume    = {4},
  number    = {3},
  year      = {1992},
  pages     = {185-211},
  ee        = {http://dx.doi.org/10.1080/09528139208953747},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{cohen2009shared,
  title={Shared logistic normal distributions for soft parameter tying in unsupervised grammar induction},
  author={Cohen, S.B. and Smith, N.A.},
  booktitle={Proceedings of Human Language Technologies: The 2009 Annual Conference of the North American Chapter of the Association for Computational Linguistics},
  pages={74--82},
  year={2009},
  organization={Association for Computational Linguistics}
}

@article{langley2000learning,
  title={Learning context-free grammars with a simplicity bias},
  author={Langley, P. and Stromsten, S.},
  journal={Machine Learning: ECML 2000},
  pages={220--228},
  year={2000},
  publisher={Springer}
}

@article{oates2006inferring,
  title={Inferring grammars for mildly context sensitive languages in polynomial-time},
  author={Oates, T. and Armstrong, T. and Bonache, L. and Atamas, M.},
  journal={Grammatical Inference: Algorithms and Applications},
  pages={137--147},
  year={2006},
  publisher={Springer}
}

@article{earley1970efficient,
  title={An efficient context-free parsing algorithm},
  author={Earley, J.},
  journal={Communications of the ACM},
  volume={13},
  number={2},
  pages={94--102},
  year={1970},
  publisher={ACM}
}

@article{sutton1999between,
  title={Between MDPs and semi-MDPs: A framework for temporal abstraction in reinforcement learning},
  author={Sutton, R.S. and Precup, D. and Singh, S.},
  journal={Artificial intelligence},
  volume={112},
  number={1},
  pages={181--211},
  year={1999},
  publisher={Citeseer}
}

@article{sadik2010modeling,
  title={Modeling high assurance agent-based Earthquake Management System using formal techniques},
  author={Sadik, S. and Rahman, A. and Ali, A. and Ahmad, H.F. and Suguri, H.},
  journal={The Journal of Supercomputing},
  volume={52},
  number={2},
  pages={97--118},
  year={2010},
  publisher={Springer}
}

@inproceedings{khosla1998human,
  title={Human-centered virtual machine of problem solving agents, software agents, intelligent agents and objects},
  author={Khosla, R.},
  booktitle={High-Assurance Systems Engineering Symposium, 1998. Proceedings. Third IEEE International},
  pages={312--319},
  year={1998},
  organization={IEEE}
}

@inproceedings{phoha1998coordination,
  title={Coordination of engineering design agents for high assurance in complex dynamic system design},
  author={Phoha, S. and Peluso, E. and Eberbach, E. and Kiraly, A.},
  booktitle={High-Assurance Systems Engineering Symposium, 1998. Proceedings. Third IEEE International},
  pages={296--303},
  organization={IEEE},
  year={1998}
}

@article{suc2004learning,
  title={Learning to Fly Simple and Robust},
  author={{\v{S}}uc, D. and Bratko, I. and Sammut, C.},
  journal={Machine Learning: ECML 2004},
  pages={407--418},
  year={2004},
  publisher={Springer}
}

@inproceedings{lyons2004towards,
  title={Towards performance guarantees for emergent behavior},
  author={Lyons, D.M. and Arkin, R.C.},
  booktitle={Robotics and Automation, 2004. Proceedings. ICRA'04. 2004 IEEE International Conference on},
  volume={4},
  pages={4153--4158},
  year={2004},
  organization={IEEE}
}

@inproceedings{judahuser,
  title={User Initiated Learning for Adaptive Interfaces},
  author={Judah, K. and Dietterich, T. and Fern, A. and Irvine, J. and Slater, M. and Tadepalli, P. and Gervasio, M. and Ellwood, C. and Jarrold, B. and Brdiczka, O. and others},
  BOOKTITLE = {{IJCAI Workshop on Intelligence and Interaction}},
  year={2009}
}

@inproceedings{garvey2009learning,
  title={Learning by demonstration to support military planning and decision making},
  author={Garvey, T. and Gervasio, M. and Lee, T. and Myers, K. and Angiolillo, C. and Gaston, M. and Knittel, J. and Kolojejchick, J.},
  booktitle={Proc. of the 21st Conference on Innovative Applications of Artificial Intelligence},
  year={2009}
}

@inproceedings{ratwani2010single,
  title={Single operator, multiple robots: an eye movement based theoretic model of operator situation awareness},
  author={Ratwani, R.M. and McCurry, J.M. and Trafton, J.G.},
  booktitle={Proceeding of the 5th ACM/IEEE international conference on Human-robot interaction},
  pages={235--242},
  year={2010},
  organization={ACM}
}

@inproceedings{boussemart2008behavioral,
  title={Behavioral recognition and prediction of an operator supervising multiple heterogeneous unmanned vehicles},
  author={Boussemart, Y. and Cummings, ML},
  booktitle={Humans operating unmanned systems},
  year={2008}
}

@article{iba1989heuristic,
  title={A heuristic approach to the discovery of macro-operators},
  author={Iba, G.A.},
  journal={Machine Learning},
  volume={3},
  number={4},
  pages={285--317},
  year={1989},
  publisher={Springer}
}


@phdthesis{pickett:2011,
  AUTHOR    = {M. Pickett},
  TITLE     = {{Towards Relational Concept Formation From Undifferentiated Sensor Data}},
  SCHOOL    = {{University of Maryland Baltimore County}},
  YEAR      = {2011},
  type      = {Doctoral dissertation},
}

@inproceedings{Armstrong07b,
	Author = {Tom Armstrong and Tim Oates},
	Booktitle = {Proceedings of the 6th {IEEE} International Conference on Development and Learning},
	Date-Added = {2007-11-30 10:25:26 -0500},
	Date-Modified = {2007-11-30 10:25:26 -0500},
	Title = {{RIPTIDE}: Segmenting Data Using Multiple Resolutions},
	Year = {2007}}

@InProceedings{robinet+lemaire:2009,
  AUTHOR = {Robinet, V. and Lemaire, B},
  TITLE = {{MDLChunker: a MDL-based Model of Word Segmentation}},
  BOOKTITLE = {{Proceedings of the 31th Annual Conference of the Cognitive Science Society}},
  YEAR      = {2009},
}

@article{Servan-schreiber90learningartificial,
    author = {Emile Servan-schreiber and John R. Anderson},
    title = {Learning artificial grammars with competitive chunking},
    journal = {Journal of Experimental Psychology: Learning, Memory, and Cognition},
    year = {1990},
    volume = {16},
    pages = {592--608}
}

@article{citeulike:1676405,
    author = {Perruchet, P. and Vintner, A.},
    citeulike-article-id = {1676405},
    citeulike-linkout-0 = {http://www.u-bourgogne.fr/LEAD/people/perruchet/pdf128Ko.pdf},
    citeulike-linkout-1 = {http://www.ingentaconnect.com/content/els/0749596x/1998/00000039/00000002/art92576},
    journal = {Journal of Memory and Language},
    keywords = {artificial-grammars, cross-situational, models},
    year = {1998},
    month = aug,
    pages = {246--263},
    posted-at = {2007-09-19 16:25:32},
    priority = {4},
    title = {{PARSER: A Model for Word Segmentation}},
    volume = {39}
}

@article{Batchelder02,
  author = {E. O. Batchelder},
  interhash = {58670efd572a253857fa3e98129207db},
  intrahash = {52ca1cf6b9b421e599235f96908ad31d},
  journal = {Cognition},
  pages = {167-206},
  title = {Bootstrapping the lexicon: A computational model of infant speech segmentation},
  volume = 83,
  year = 2002,
  timestamp = {2008-09-16T23:39:07.000+0200},
  keywords = {devo},
  added-at = {2008-09-16T23:39:07.000+0200},
  description = {CCNLab BibTeX},
}

@article{citeulike:4208032,
    author = {Gobet, F. and Lane, P. and Croker, S. and Cheng, P. and Jones, G. and Oliver, I. and Pine, J.},
    citeulike-article-id = {4208032},
    citeulike-linkout-0 = {http://dx.doi.org/10.1016/S1364-6613(00)01662-4},
    citeulike-linkout-1 = {http://linkinghub.elsevier.com/retrieve/pii/S1364661300016624},
    day = {01},
    doi = {10.1016/S1364-6613(00)01662-4},
    issn = {13646613},
    journal = {Trends in Cognitive Sciences},
    keywords = {chunking, information\_processing},
    month = jun,
    number = {6},
    pages = {236--243},
    posted-at = {2009-03-23 02:04:05},
    priority = {2},
    title = {{Chunking Mechanisms in Human Learning}},
    volume = {5},
    year = {2001}
}


@inproceedings{Edelman04bridgingcomputational,
    author = {Shimon Edelman and Zach Solan and David Horn and Eytan Ruppin},
    title = {Bridging Computational, Formal and Psycholinguistic Approaches to Language},
    booktitle = {In Proc. of The 26th Conference of The Cognitive Science Society},
    year = {2004},
}

@Article{little:1955,
  AUTHOR    = {Little, J.\ D.\ C.},
  TITLE     = {{The Use of Storage Water in Hydroelectric Systems}},
  JOURNAL   = {Opns Res.},
  PAGES     = {187-197},
  YEAR      = {1955},
}

@inproceedings{DBLP:conf/colt/Schmidhuber02,
  author    = {J{\"u}rgen Schmidhuber},
  title     = {The Speed Prior: A New Simplicity Measure Yielding Near-Optimal
               Computable Predictions},
  booktitle = {COLT},
  year      = {2002},
  pages     = {216-228},
  ee        = {http://link.springer.de/link/service/series/0558/bibs/2375/23750216.htm},
  crossref  = {DBLP:conf/colt/2002},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/colt/2002,
  editor    = {Jyrki Kivinen and
               Robert H. Sloan},
  title     = {Computational Learning Theory, 15th Annual Conference on
               Computational Learning Theory, COLT 2002, Sydney, Australia,
               July 8-10, 2002, Proceedings},
  booktitle = {COLT},
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {2375},
  year      = {2002},
  isbn      = {3-540-43836-X},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{DBLP:journals/tit/ZivL77,
  author    = {Jacob Ziv and
               Abraham Lempel},
  title     = {A Universal Algorithm for Sequential Data Compression},
  journal   = {IEEE Transactions on Information Theory},
  volume    = {23},
  number    = {3},
  year      = {1977},
  pages     = {337-343},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@Article{zhu:2008,
  AUTHOR    = {Xiaojin Zhu},
  TITLE     = {{Semi-Supervised Learning Literature Survey}},
  JOURNAL   = {Technical Report, University of Wisconsin Madison, Computer Sciences TR 1530},
  YEAR      = {2008},
}

@INPROCEEDINGS{Zhou07semi-supervisedlearning,
    author = {Zhi-hua Zhou and De-chuan Zhan and Qiang Yang},
    title = {Semi-supervised learning with very few labeled training examples},
    booktitle = {Twenty-Second AAAI Conference on Artificial Intelligence (AAAI-07},
    year = {2007},
    pages = {675--680}
}

@inproceedings{Meraz:2004:PSO:1018417.1019310,
 author = {Meraz, Richard F. and He, Xiaofeng and Ding, Chris H. Q. and Holbrook, Stephen R.},
 title = {Positive Sample Only Learning (PSOL) for Predicting RNA Genes in E. coli},
 booktitle = {Proceedings of the 2004 IEEE Computational Systems Bioinformatics Conference},
 series = {CSB '04},
 year = {2004},
 isbn = {0-7695-2194-0},
 pages = {535--538},
 numpages = {4},
 doi = {http://dx.doi.org/10.1109/CSB.2004.129},
 acmid = {1019310},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}


@inproceedings{elkan.kdd08,
  title     = "Learning Classifiers from Only Positive and Unlabeled Data",
  author    = "C. Elkan and K. Noto",
  booktitle = "Proceedings of the 14th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining (KDD 2008)",
  pages     = "213--220",
  year      = "2008"
}


@inproceedings{DBLP:conf/ilp/Muggleton96,
  author    = {Stephen Muggleton},
  title     = {Learning from Positive Data},
  booktitle = {Inductive Logic Programming Workshop},
  year      = {1996},
  pages     = {358-376},
  crossref  = {DBLP:conf/ilp/1996},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@proceedings{DBLP:conf/ilp/1996,
  editor    = {Stephen Muggleton},
  title     = {Inductive Logic Programming, 6th International Workshop,
               ILP-96, Stockholm, Sweden, August 26-28, 1996, Selected
               Papers},
  booktitle = {ILP},
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {1314},
  year      = {1997},
  isbn      = {3-540-63494-0},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{Feifei06,
    address = {Washington, DC, USA},
    author = {Fei-Fei, Li and Fergus, R. and Perona, P.},
    citeulike-article-id = {518788},
    citeulike-linkout-0 = {http://portal.acm.org/citation.cfm?id=1115692.1115783},
    citeulike-linkout-1 = {http://dblp.uni-trier.de/rec/bibtex/journals/pami/Fei-FeiFP06},
    citeulike-linkout-2 = {http://dx.doi.org/10.1109/TPAMI.2006.79},
    citeulike-linkout-3 = {http://ieeexplore.ieee.org/xpls/abs\_all.jsp?arnumber=1597116},
    doi = {10.1109/TPAMI.2006.79},
    issn = {0162-8828},
    journal = {IEEE Trans. Pattern Anal. Mach. Intell.},
    keywords = {image\_classification, learning},
    number = {4},
    pages = {594--611},
    posted-at = {2007-06-20 17:28:17},
    priority = {2},
    publisher = {IEEE Computer Society},
    title = {{One-Shot Learning of Object Categories}},
    volume = {28},
    year = {2006}
}


@article{citeulike:7874864Muggleton,
    author = {Muggleton, S.},
    citeulike-article-id = {7874864},
    citeulike-linkout-0 = {http://dx.doi.org/10.1016/0743-1066(94)90035-3},
    citeulike-linkout-1 = {http://linkinghub.elsevier.com/retrieve/pii/0743-1066(94)90035-3},
    doi = {10.1016/0743-1066(94)90035-3},
    issn = {07431066},
    journal = {The Journal of Logic Programming},
    month = may,
    pages = {629--679},
    posted-at = {2010-09-22 10:53:23},
    priority = {2},
    title = {{Inductive Logic Programming: Theory and methods}},
    volume = {19-20},
    year = {1994}
}

@article{marcus:1992,
  author = {Gary F. Marcus},
  journal = {Cognition},
  title = {{Negative Evidence in Language Acquisition}},
  month = {July},
  year = 1993,
}

@article{rohde:1999,
  author = {Douglas L. T. Rohde and David C. Plaut},
  journal = {Cognition},
  title = {{Language Acquisition in the Absence of Explicit Negative Evidence: How Important is Starting Small?}},
  month = {June},
  year = 1999,
}

@book{citeulike:chomsky3360687,
    author = {Chomsky, Noam},
    citeulike-article-id = {3360687},
    day = {04},
    howpublished = {Paperback},
    isbn = {0231132719},
    keywords = {80, brain, modular, modularity},
    month = may,
    posted-at = {2008-09-30 20:37:10},
    priority = {2},
    publisher = {Columbia University Press},
    title = {{Rules and Representations (Columbia Classics in Philosophy)}},
    year = {2005}
}



@article{Gold67,
  author = {E. Mark Gold},
  interhash = {ef3b6d7384405e033e133ce6c73dc2f9},
  intrahash = {1d4a44d1927da0811acd3caab51d5824},
  journal = {Information and Control},
  number = 5,
  pages = {447--474},
  title = {Language Identification in the Limit},
  volume = 10,
  year = 1967,
  keywords = {article identification_in_the_limit induction machine_learning seminal_paper},
  added-at = {2010-04-21T21:55:33.000+0200},
  description = {golds seminal paper on inductive inference},
}


@inproceedings{Raina+etal07:selfTaughtLearning,
	title = {Self-taught Learning: Transfer Learning from Unlabeled Data},
	author = {Raina, Rajat and Battle, Alexis and Lee, Honglak and Packer, Benjamin and Ng, Andrew Y.},
	booktitle = {Proceedings of the 24th International Conference on Machine learning},
	year = {2007},
	pages = {759--766},
}

@article{Garson:1991:INC:129449.129452,
 author = {Garson, G. David},
 title = {{Interpreting Neural-Network Connection Weights}},
 journal = {AI Expert},
 volume = {6},
 issue = {4},
 month = {April},
 year = {1991},
 issn = {0888-3785},
 pages = {46--51},
 numpages = {6},
 acmid = {129452},
 publisher = {Miller Freeman, Inc.},
 address = {San Francisco, CA, USA},
}

@inproceedings{DBLP:conf/fgr/Blanz06,
  author    = {Volker Blanz},
  title     = {Face Recognition based on a 3D Morphable Model},
  booktitle = {FG},
  year      = {2006},
  pages     = {617-624},
  ee        = {http://doi.ieeecomputersociety.org/10.1109/FGR.2006.42},
  crossref  = {DBLP:conf/fgr/2006},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@proceedings{DBLP:conf/fgr/2006,
  editor    = {Mark Nixon and Josef Kittler},
  title     = {Seventh IEEE International Conference on Automatic Face
               and Gesture Recognition (FG 2006), 10-12 April 2006, Southampton,
               UK},
  booktitle = {FG},
  publisher = {IEEE Computer Society},
  year      = {2006},
  isbn      = {0-7695-2503-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@inproceedings{DBLP:conf/ibpria/ChorasM07,
  author    = {Michal Choras and
               Piotr Mroczkowski},
  title     = {{Recognizing Individual Typing Patterns}},
  booktitle = {IbPRIA (2)},
  year      = {2007},
  pages     = {323-330},
  ee        = {http://dx.doi.org/10.1007/978-3-540-72849-8_41},
  crossref  = {DBLP:conf/ibpria/2007-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@proceedings{DBLP:conf/ibpria/2007-2,
  editor    = {Joan Mart\'{\i} and
               Jos{\'e}-Miguel Bened\'{\i} and
               Ana Maria Mendon\c{c}a and
               Joan Serrat},
  title     = {Pattern Recognition and Image Analysis, Third Iberian Conference,
               IbPRIA 2007, Girona, Spain, June 6-8, 2007, Proceedings,
               Part II},
  booktitle = {IbPRIA (2)},
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {4478},
  year      = {2007},
  isbn      = {978-3-540-72848-1},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{citeulike:1068501,
    author = {Przulj, Natasa},
    citeulike-article-id = {1068501},
    day = {15},
    doi = {10.1093/bioinformatics/btl301},
    issn = {1367-4803},
    journal = {Bioinformatics},
    month = jan,
    number = {2},
    pages = {e177--e183},
    posted-at = {2010-06-29 21:15:09},
    priority = {2},
    publisher = {Oxford University Press},
    title = {{Biological Network Comparison Using Graphlet Degree Distribution}},
    volume = {23},
    year = {2007}
}

@article{steyvers2005large,
  title={The Large-Scale Structure of Semantic Networks: Statistical Analyses and a Model of Semantic Growth},
  author={Steyvers, Mark and Tenenbaum, Joshua B},
  journal={Cognitive science},
  volume={29},
  number={1},
  pages={41--78},
  year={2005},
  publisher={Wiley Online Library}
}

@inproceedings {SheVisPet2009,
        title = {{Efficient Graphlet Kernels for Large Graph Comparison}},
        booktitle = {{Int. Conf. on AI \& Stats.}},
        year = {2009},
        author = {Nino Shervashidze and Vishwanathan, SVN and Tobias Petri and Kurt Mehlhorn and Karsten Borgwardt},
        address = {}
}

@inproceedings{pearl85bayesian,
    author = {Pearl, Judea},
    booktitle = {Proceedings of the 7th Conference of the Cognitive Science Society, University of California, Irvine},
    citeulike-article-id = {1911949},
    citeulike-linkout-0 = {http://www.amazon.com/Bayesian-networks-self-activated-evidential-University/dp/B00071DFAE},
    day = {15--17},
    keywords = {bayesian, pearl},
    month = {August},
    pages = {329--334},
    posted-at = {2007-11-14 03:23:00},
    priority = {1},
    title = {{Bayesian networks: A model of self-activated memory for evidential reasoning}},
    year = {1985}
}


@incollection {stolcke:1994,
   author = {Stolcke, Andreas and Omohundro, Stephen},
   affiliation = {International Computer Science Institute 1947 Center St., Suite 600 94707 Berkeley CA 1947 Center St., Suite 600 94707 Berkeley CA},
   title = {{Inducing Probabilistic Grammars by Bayesian Model Merging}},
   booktitle = {Grammatical Inference and Applications},
   series = {Lecture Notes in Computer Science},
   editor = {Carrasco, Rafael and Oncina, Jose},
   publisher = {Springer Berlin / Heidelberg},
   isbn = {},
   pages = {106-118},
   volume = {862},
   year = {1994}
}

@article{hummel+holyoak:2005,
    author = {John E. Hummel and Keith J. Holyoak},
    journal = {Current Directions in Psychological Science},
    month = {June},
    number = {3},
    pages = {153--157},
    title = {{Relational Reasoning in a Neurally Plausible Cognitive Architecture: An Overview of the LISA Project}},
    volume = {14},
    year = {2005}
}

@article{Friedman03,
    author = {Friedman, Nir and Koller, Daphne},
    citeulike-article-id = {404290},
    citeulike-linkout-0 = {http://www.ingentaconnect.com/content/klu/mach/2003/00000050/F0020001/05096739},
    issn = {0885-6125},
    journal = {Machine Learning},
    keywords = {graphical\_models, learning},
    month = {January},
    number = {1-2},
    pages = {95--125},
    posted-at = {2008-10-30 16:46:22},
    priority = {1},
    publisher = {Springer Netherlands},
    title = {{Being Bayesian About Network Structure. A Bayesian Approach to Structure Discovery in Bayesian Networks}},
    volume = {50},
    year = {2003}
}

@ARTICLE{Forbus98analogyjust,
    author = {Kenneth D. Forbus and Dedre Gentner and Arthur B. Markman and Ronald W. Ferguson},
    title = {{Analogy Just Looks Like High Level Perception: Why a Domain-General Approach to Analogical Mapping is Right}},
    journal = {Journal of experimental and Theoretical Artificial Intelligence},
    year = {1998},
    volume = {10},
    pages = {231--257}
}

@book{Kanerva:1988:SDM:534853,
 author = {Kanerva, Pentti},
 title = {{Sparse Distributed Memory}},
 year = {1988},
 isbn = {0262111322},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
}

@article{kemp:theory-formation,
    author = {Kemp, Charles and Tenenbaum, Joshua B. and Niyogi, Sourabh and Griffiths, Thomas L.},
    citeulike-article-id = {6212252},
    day = {04},
    doi = {10.1016/j.cognition.2009.09.003},
    issn = {1873-7838},
    journal = {Cognition},
    keywords = {bayesian, psych, smrf\_related, theory\_formation},
    month = {February},
    number = {2},
    pages = {165--196},
    posted-at = {2010-06-22 16:59:59},
    priority = {2},
    title = {{A probabilistic model of theory formation.}},
    volume = {114},
    year = {2010}
}

@article{tenenbaum+kemp:2008,
  address = {Department of Psychology, Carnegie Mellon University, 5000 Forbes Avenue, Pittsburgh, PA 15213.},
  author = {Charles Kemp and Joshua B. Tenenbaum},
  journal = {Proceedings of the National Academy of Sciences of the United States of America},
  title = {{The discovery of structural form.}},
  year = 2008,
  keywords = {bayesian concept constraints imported learning structure unsupervised},
  added-at = {2009-03-06T14:41:46.000+0100},
  posted-at = {2008-08-07 21:40:11},
  issn = {1091-6490},
  priority = {2},
  citeulike-article-id = {3080763},
  doi = {http://dx.doi.org/10.1073/pnas.0802631105},
  month = {July},
}

@article{schmidt2009distilling,
  title={{Distilling Free-Form Natural Laws from Experimental Data}},
  author={Schmidt, Michael and Lipson, Hod},
  journal={Science},
  volume={324},
  number={5923},
  pages={81--85},
  year={2009},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{Lowe:1999:ORL:850924.851523,
 author = {Lowe, David G.},
 title = {Object Recognition from Local Scale-Invariant Features},
 booktitle = {Proceedings of the International Conference on Computer Vision-Volume 2 - Volume 2},
 series = {ICCV '99},
 year = {1999},
 isbn = {0-7695-0164-8},
 pages = {1150--},
 acmid = {851523},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
}

@article{DBLP:journals/artmed/Kuipers08,
  author    = {Benjamin Kuipers},
  title     = {{Drinking from the Firehose of Experience}},
  journal   = {Artificial Intelligence in Medicine},
  volume    = {44},
  number    = {2},
  year      = {2008},
  pages     = {155-170},
  ee        = {http://dx.doi.org/10.1016/j.artmed.2008.07.010},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@Article{george:2008,
  AUTHOR    = {Dileep George},
  TITLE     = {{How the Brain Might Work: A Hierarchical and Temporal Model for Learning and Recognition}},
  JOURNAL   = {PhD Thesis, Stanford University},
  YEAR      = {2008},
}

@article{george+hawkins:5915686,
    author = {George, Dileep and Hawkins, Jeff},
    citeulike-article-id = {5915686},
    citeulike-linkout-0 = {http://dx.doi.org/10.1371/journal.pcbi.1000532},
    citeulike-linkout-1 = {http://view.ncbi.nlm.nih.gov/pubmed/19816557},
    citeulike-linkout-2 = {http://www.hubmed.org/display.cgi?uids=19816557},
    day = {9},
    doi = {10.1371/journal.pcbi.1000532},
    issn = {1553-7358},
    journal = {PLoS Comput Biol},
    keywords = {hierarchical-model},
    month = {October},
    number = {10},
    posted-at = {2010-02-12 23:54:52},
    priority = {2},
    publisher = {Public Library of Science},
    title = {{Towards a Mathematical Theory of Cortical Micro-circuits}},
    volume = {5},
    year = {2009}
}

@book{Drescher:1991:MMC:113149,
 author = {Drescher, Gary L.},
 title = {{Made-Up Minds: A Constructivist Approach to Artificial Intelligence}},
 year = {1991},
 isbn = {0-262-04120-0},
 publisher = {MIT Press},
 address = {Cambridge, MA, USA},
}

@Article{getoor:jmlr02,
  author       = "Getoor, Lise and Friedman, Nir and Koller, Daphne and Taskar, Benjamin",
  title        = "Learning Probabilistic Models of Link Structure",
  journal      = "Journal of Machine Learning Research",
  volume       = "3",
  pages        = "679- -707",
  year         = "2002",
}
@InProceedings{getoor:icml01,
  author       = "Getoor, Lise and Friedman, Nir and Koller, Daphne and Taskar, Benjamin",
  title        = "Learning Probabilistic Models of Relational Structure",
  booktitle    = "Proceedings of International Conference on Machine Learning (ICML)",
  year         = "2001",
}
@InCollection{getoor:rdm-book01,
  author       = "Getoor, Lise and Friedman, Nir and Koller, Daphne and Pfeffer, Avi",
  title        = "Learning Probabilistic Relational Models",
  booktitle    = "Relational Data Mining",
  year         = "2001",
  editor       = "S. Dzeroski and N. Lavrac",
  publisher    = "Springer-Verlag",
}


@InProceedings{pickett+miner+oates:2008,
  AUTHOR    = {M. Pickett and D. Miner and T. Oates},
  TITLE     = {{Essential Phenomena of General Intelligence}},
  BOOKTITLE = {{Proceedings of The First Conference on Artificial General Intelligence}},
  YEAR      = {2008},
}
@InProceedings{pickett+miner:2007,
  AUTHOR    = {M. Pickett and D. Miner},
  TITLE     = {{Representation Change in The Marchitecture}},
  BOOKTITLE = {{Working Notes of the AAAI Fall Symposium on Representation Change}},
  YEAR      = {2007},
}
@InProceedings{pickett+miner+oates:2007,
  AUTHOR    = {M. Pickett and D. Miner and T. Oates},
  TITLE     = {{A Gauntlet for Evaluating Cognitive Architectures}},
  BOOKTITLE = {{Working Notes of the AAAI Workshop on Evaluating Architectures for Intelligence}},
  YEAR      = {2007},
}
@InProceedings{pickett+oates:2007,
  AUTHOR    = {M. Pickett and T. Oates},
  TITLE     = {{The Marchitecture: A Cognitive Architecture for a Robot Baby}},
  BOOKTITLE = {{Proceedings of the 22nd AAAI Conference on Artificial Intelligence (AAAI-07)}},
  NOTE      = {Student abstract and poster},
  YEAR      = {2007},
}
@InProceedings{pickett:2007a,
  AUTHOR    = {M. Pickett},
  TITLE     = {{The \"Ubercruncher: Concept Formation by Analogy Discovery}},
  BOOKTITLE = {{Proceedings of the 22nd AAAI Conference on Artificial Intelligence (AAAI-07), Doctoral Consortium}},
  YEAR      = {2007},
}
@InProceedings{pickett:2007,
  AUTHOR    = {M. Pickett},
  TITLE     = {{Using Analogy Discovery to Create Abstractions}},
  BOOKTITLE = {{Proceedings of the 7th International Symposium on Abstraction, Reformulation and Approximation (SARA 2007)}},
  YEAR      = {2007},
  SERIES    = {Lecture Notes in Artificial Intelligence},
  PUBLISHER = {Springer Verlag},
}
@InProceedings{chaddock+pickett+armstrong+oates:2007,
  AUTHOR    = {G. Chaddock and M. Pickett and T. Armstrong and T. Oates},
  TITLE     = {{Models of Strategic Deficiency and Poker}},
  BOOKTITLE = {{Working Notes of the AAAI Workshop on Plan, Activity, and Intent Recognition (PAIR)}},
  YEAR      = {2007},
}
@InProceedings{pickett+oates:2005,
  AUTHOR    = {M. Pickett and T. Oates},
  TITLE     = {{The Cruncher: Automatic Concept Formation Using Minimum Description Length}},
  BOOKTITLE = {{Proceedings of the 6th International Symposium on Abstraction, Reformulation and Approximation (SARA 2005)}},
  YEAR      = {2005},
  SERIES    = {Lecture Notes in Artificial Intelligence},
  PUBLISHER = {Springer Verlag},
}
@techreport{berry+ko+moy+pickett+smrcka+turnley+wu:2003,
  AUTHOR    = {N. Berry and T. Ko and T. Moy and M. Pickett and J. Smrcka and J. Turnley and B. Wu},
  TITLE     = {{Computational Social Dynamic Modeling of Group Recruitment}},
  type     = {Sandia Report},
  number   = {SAND2003-8754},
  INSTITUTION = {Sandia National Laboratories},
  YEAR      = {2003},
}
@InProceedings{pickett:2002,
  AUTHOR    = {M. Pickett},
  TITLE     = {{Research Summary}},
  BOOKTITLE = {{Proceedings of the 5th International Symposium on Abstraction, Reformulation and Approximation (SARA 2002)}},
  YEAR      = {2002},
  SERIES    = {Lecture Notes in Artificial Intelligence},
  PUBLISHER = {Springer Verlag},
}
@InProceedings{pickett+barto:2002,
  AUTHOR    = {M. Pickett and A. Barto},
  TITLE     = {{PolicyBlocks: An Algorithm For Creating Useful Macro-Actions in Reinforcement Learning}},
  BOOKTITLE = {{Proceedings of the International Conference on Machine Learning}},
  YEAR      = {2002},
}
@Book{pickett:2006,
  AUTHOR    = {M. Pickett},
  PUBLISHER = {Lulu},
  ISBN      = {978-0-557-03376-8},
  TITLE     = {{Europe Debris: The Epic of Gabe and Marc in Europe}},
  YEAR      = {2006},
}
@Article{vondermalsburg:1999,
  AUTHOR    = {C. von der Malsburg},
  TITLE     = {{The What and Why of Binding: The Modeler's Perspective}},
  JOURNAL   = {Neuron},
  VOLUME    = {24},
  PAGES     = {95-104},
  YEAR      = {1999},
}
@Book{plato:VII:-360,
  AUTHOR    = {Plato},
  TITLE     = {{The Republic, Book VII}},
  PUBLISHER = {(Public domain)},
  YEAR      = {360 BC},
}
@Book{plato:meno:-387,
  AUTHOR    = {Plato},
  TITLE     = {{The Meno}},
  PUBLISHER = {(Public domain)},
  YEAR      = {387 BC},
}
@Article{lynch:2004,
  AUTHOR    = {M. Lynch},
  TITLE     = {{Long-term Potentiation and Memory}},
  JOURNAL   = {Physiol. Rev.},
  VOLUME    = {84},
  PAGES     = {87-136},
  YEAR      = {2004},
}
@Article{mccarthy+hayes:1969,
  AUTHOR    = {J. McCarthy and P. J. Hayes},
  TITLE     = {{Some Philosophical Problems from the Standpoint of Artificial Intelligence}},
  JOURNAL   = {Machine Intelligence},
  VOLUME    = {4},
  PAGES     = {463-502},
  YEAR      = {1969},
}
@Book{dawkins:1976,
  AUTHOR    = {R. Dawkins},
  TITLE     = {{The Selfish Gene}},
  PUBLISHER = {Oxford University Press},
  ADDRESS   = {Oxford, England},
  YEAR      = {1976},
}
@Book{hutter:2004,
  AUTHOR    = {M. Hutter},
  TITLE     = {{Universal Artificial Intelligence: Sequential Decisions based on Algorithmic Probability}},
  SERIES    = {EATCS},
  PUBLISHER = {Springer},
  ADDRESS   = {Berlin},
  YEAR      = {2004},
}
@Book{pearl:2000,
  AUTHOR    = {J. Pearl},
  TITLE     = {{Causality}},
  PUBLISHER = {Cambridge University Press},
  YEAR      = {2000},
}
@Book{barthorp:1980,
  AUTHOR    = {M. Barthorp},
  PUBLISHER = {Blandford Press},
  TITLE     = {{The Zulu War}},
  YEAR      = {1980},
  ADDRESS   = {Dorset, England},
}
@Book{polanyi:1967,
  AUTHOR    = {M. Polanyi},
  PUBLISHER = {Anchor Books},
  TITLE     = {{The Tacit Dimension}},
  YEAR      = {1967},
  ADDRESS   = {New York},
}
@InProceedings{witbrock+matuszek+brusseau+kahlert+fraser+lenat:2005,
  AUTHOR    = {M. Witbrock  and C. Matuszek and A. Brusseau and  R. C. Kahlert and C.B. Fraser and D. Lenat},
  TITLE     = {{Knowledge Begets Knowledge: Steps towards Assisted Knowledge Acquisition in Cyc}},
  BOOKTITLE = {{Papers from the 2005 AAAI Spring Symposium on Knowledge Collection from Volunteer Contributors (KCVC)}},
  YEAR      = {2005},
  PAGES     = {99-105},
  ADDRESS   = {Stanford, California},
}
@Article{harnad:1990,
  AUTHOR    = {S. Harnad},
  TITLE     = {{The Symbol Grounding Problem}},
  JOURNAL   = {Physica D},
  VOLUME    = {42},
  PAGES     = {335-346},
  YEAR      = {1990},
}
@Book{langley+laird:2002,
  AUTHOR    = {P. Langley and J. Laird},
  PUBLISHER = {Manuscript},
  TITLE     = {{Cognitive Architectures: Research Issues and Challenges}},
  YEAR      = {2002},
}
@Book{anderson:1993,
  AUTHOR    = {J. R. Anderson},
  PUBLISHER = {Lawrence Erlbaum Associates},
  TITLE     = {{Rules of the Mind}},
  YEAR      = {1993},
  ADDRESS   = {Hillsdale, NJ},
}
@Book{anderson:1983,
  AUTHOR    = {J. R. Anderson},
  PUBLISHER = {Harvard University Press},
  TITLE     = {{The Architecture of Cognition}},
  YEAR      = {1983},
  ADDRESS   = {Cambridge, MA},
}
@Book{rosenbloom+laird+newell:1993,
  AUTHOR    = {P. Rosenbloom and J. Laird and A. Newell},
  PUBLISHER = {MIT Press},
  TITLE     = {{The SOAR papers: research on integrated intelligence}},
  YEAR      = {1993},
  ADDRESS   = {Cambridge, MA},
}
@InProceedings{cohen+oates+beal+adams:2002,
  AUTHOR    = {P. Cohen and T. Oates and C. Beal and N. Adams},
  TITLE     = {{Contentful Mental States for Robot Baby}},
  BOOKTITLE = {{Proceedings of the 18th National Conference on Artificial Intelligence}},
  YEAR      = {2002},
}
@Book{malthus:1798,
  AUTHOR    = {T. R. Malthus},
  PUBLISHER = {J. Johnson},
  TITLE     = {{An Essay on the Principle of Population}},
  YEAR      = {1798},
}
@Article{shannon:1948,
  AUTHOR    = {C. E. Shannon},
  TITLE     = {{A Mathematical Theory of Communication}},
  JOURNAL   = {Bell System Technical Journal},
  VOLUME    = {27},
  PAGES     = {379-423 and 623-656},
  YEAR      = {1948},
}
@Article{whorf:1939,
  AUTHOR    = {B. L. Whorf},
  TITLE     = {{The Relation of Habitual Thought and Behavior to Language}},
  YEAR      = {1939},
}
@Book{pinker:1999,
  AUTHOR    = {S. Pinker},
  PUBLISHER = {Basic Books},
  TITLE     = {{Words and Rules: The Ingredients of Language}},
  YEAR      = {1999},
}
@Book{pinker:1994,
  AUTHOR    = {S. Pinker},
  PUBLISHER = {Harper Perennial Modern Classics},
  TITLE     = {{The Language Instinct}},
  YEAR      = {1994},
}
@Book{fodor:1975,
  AUTHOR    = {J. Fodor},
  PUBLISHER = {Harvard University Press},
  TITLE     = {{The Language of Thought}},
  YEAR      = {1975},
}
@Article{mandler:1992,
  AUTHOR    = {J. M. Mandler},
  TITLE     = {{How to Build a Baby II: Conceptual Primitives}},
  JOURNAL   = {Psychological Review},
  VOLUME    = {99},
  PAGES     = {587-604},
  YEAR      = {1992},
}
@Book{diamond:1999,
  AUTHOR    = {J. Diamond},
  PUBLISHER = {W. W. Norton and Company},
  TITLE     = {{Guns, Germs, and Steel: The Fates of Human Societies}},
  YEAR      = {1999},
}
@Book{morrison+morrison:1994,
  AUTHOR    = {P. Morrison and P. Morrison},
  PUBLISHER = {W. H. Freeman and Company},
  TITLE     = {{Powers of Ten (Revised edition)}},
  YEAR      = {1994},
}
@Book{lenat+guha:1990,
  AUTHOR    = {D. Lenat and R. V. Guha},
  PUBLISHER = {Addison-Wesley},
  TITLE     = {{Building Large Knowledge-Based Systems: Representation and Inference in the Cyc Project}},
  YEAR      = {1990},
}
@Book{attenborough:1995,
  AUTHOR    = {D. Attenborough},
  PUBLISHER = {Princeton University Press},
  TITLE     = {{The Private Life of Plants}},
  YEAR      = {1995},
}
@Book{holldobler+wilson:1998,
  AUTHOR    = {B. H\"olldobler and E. O. Wilson},
  PUBLISHER = {Belknap Press},
  TITLE     = {{Journey to the Ants: A Story of Scientific Exploration}},
  YEAR      = {1998},
}
@Book{wilson:1998,
  AUTHOR    = {E. O. Wilson},
  PUBLISHER = {Vintage},
  TITLE     = {{Consilience: The Unity of Knowledge}},
  YEAR      = {1998},
}
@Book{ridley:1995,
  AUTHOR    = {M. Ridley},
  PUBLISHER = {Harper Perennial},
  TITLE     = {{The Red Queen: Sex and the Evolution of Human Nature}},
  YEAR      = {1995},
}
@Book{miller:2001,
  AUTHOR    = {G. Miller},
  PUBLISHER = {Anchor},
  TITLE     = {{The Mating Mind: How Sexual Choice Shaped the Evolution of Human Nature}},
  YEAR      = {2001},
}
@Article{leibenstein:1950,
  AUTHOR    = {H. Leibenstein},
  TITLE     = {{Bandwagon, Snob, and Veblen Effects in the Theory of Consumers' Demand}},
  JOURNAL   = {Quarterly Journal of Economics},
  VOLUME    = {64},
  PAGES     = {183-207},
  YEAR      = {1950},
}
@Article{eysenck:1991,
  AUTHOR    = {H. J. Eysenck},
  TITLE     = {{Dimensions of Personality: 5 or 3? Criteria for a Taxonomic Paradigm}},
  JOURNAL   = {Personality and Individual Differences},
  VOLUME    = {12},
  PAGES     = {773-90},
  YEAR      = {1991},
}
@Book{dabbs+dabbs:2000,
  AUTHOR    = {J. M. Dabbs and M. G. Dabbs},
  PUBLISHER = {McGraw-Hill Companies},
  TITLE     = {{Heroes, Rogues, and Lovers: Testosterone and Behavior}},
  YEAR      = {2000},
}
@Article{john+srivastava:1999,
  AUTHOR    = {O. P. John and S. Srivastava},
  TITLE     = {{The Big-Five Trait Taxonomy: History, Measurement, and Theoretical Perspectives}},
  JOURNAL   = {Handbook of Personality Theory and Research},
  VOLUME    = {2},
  PAGES     = {102-138},
  YEAR      = {1999},
  EDITOR    = {A. Pervin and O. P. John},
  PUBLISHER = {Guilford Press},
  ADDRESS   = {New York},
}
@Book{levitt+dubner:2005,
  AUTHOR    = {S. Levitt and S. Dubner},
  PUBLISHER = {William Morrow},
  TITLE     = {{Freakonomics: A Rogue Economist Explores the Hidden Side of Everything}},
  YEAR      = {2005},
}
@Book{long:2001,
  AUTHOR    = {E. Long},
  PUBLISHER = {Infinity Publishing},
  TITLE     = {{Chimpanzees Don't Wear Pants: A Retired Psychiatrist Takes a Second Look at Human Nature}},
  YEAR      = {2001},
}
@Book{wrangham+peterson:1996,
  AUTHOR    = {R. Wrangham and D. Peterson},
  PUBLISHER = {Mariner Books},
  TITLE     = {{Demonic Males: Apes and the Origins of Human Violence}},
  YEAR      = {1996},
}
@Book{dewaal:1982,
  AUTHOR    = {F. de Waal},
  PUBLISHER = {Johns Hopkins University Press},
  TITLE     = {{Chimpanzee Politics: Power and Sex among Apes}},
  YEAR      = {1982},
}
@Book{dewaal:2001,
  AUTHOR    = {F. de Waal},
  PUBLISHER = {Basic Books},
  TITLE     = {{The Ape and the Sushi Master: Cultural Reflections of a Primatologist}},
  YEAR      = {2001},
}
@Article{sun:2004,
  AUTHOR    = {R. Sun},
  TITLE     = {{Desiderata for Cognitive Architectures}},
  JOURNAL   = {Philosophical Psychology},
  VOLUME    = {17},
  NUMBER    = {3},
  PAGES     = {341-373},
  YEAR      = {2004},
}
@Misc{winston:1999,
  AUTHOR    = {P. H. Winston},
  YEAR      = {1999},
  TITLE     = {{Why I Am Optimistic}},
}
@Book{kuhn:1962,
  AUTHOR    = {T. S. Kuhn},
  PUBLISHER = {University Of Chicago Press},
  TITLE     = {{The Structure of Scientific Revolutions}},
  YEAR      = {1962},
}
@Article{nilsson:1995,
  AUTHOR    = {N. J. Nilsson},
  TITLE     = {{Eye on the Prize}},
  JOURNAL   = {AI Magazine},
  VOLUME    = {16},
  NUMBER    = {2},
  PAGES     = {9-17},
  YEAR      = {1995},
}
@InProceedings{yan+han:2002,
  AUTHOR    = {X. Yan and J. Han},
  TITLE     = {{gSpan: Graph-based substructure pattern mining}},
  BOOKTITLE = {{Proceedings of the 2002 IEEE International Conference on Data Mining (ICDM 2002)}},
  YEAR      = {2002},
}
@Misc{dumbill:2002,
  AUTHOR    = {E. Dumbill},
  YEAR      = {2002},
  TITLE     = {{XML Watch: Finding friends with XML and RDF: The Friend-of-a-Friend vocabulary can make it easier to manage online communities}},
}
@InProceedings{ding+zhou+finin+joshi:2005,
  AUTHOR    = {L. Ding and L. Zhou and T. Finin and A. Joshi},
  TITLE     = {{How the Semantic Web is Being Used: An Analysis of FOAF}},
  BOOKTITLE = {{38th Int. Conf. on System Sciences}},
  YEAR      = {2005},
}
@InProceedings{gal+modica+jamil:2004,
  AUTHOR    = {A. Gal and G. Modica and H. Jamil},
  TITLE     = {{OntoBuilder: Fully Automatic Extraction and Consolidation of Ontologies from Web Sources}},
  BOOKTITLE = {{ICDE '04: Proceedings of the 20th International Conference on Data Engineering}},
  YEAR      = {2004},
  ISBN      = {0-7695-2065-0},
  PAGES     = {853},
  PUBLISHER = {IEEE Computer Society},
  ADDRESS   = {Washington, DC, USA},
}
@InProceedings{velardi+fabriani+missikoff:2001,
  AUTHOR    = {P. Velardi and P. Fabriani and M. Missikoff},
  TITLE     = {{Using text processing techniques to automatically enrich a domain ontology}},
  BOOKTITLE = {{FOIS '01: Proceedings of the International Conference on Formal Ontology in Information Systems}},
  YEAR      = {2001},
  ISBN      = {1-58113-377-4},
  PAGES     = {270-284},
  LOCATION  = {Ogunquit, Maine, USA},
  DOI       = {http://doi.acm.org/10.1145/505168.505194},
  PUBLISHER = {ACM Press},
  ADDRESS   = {New York, NY, USA},
}
@InProceedings{oates+doshi+huang:2003,
  AUTHOR    = {T. Oates and S. Doshi and F. Huang},
  TITLE     = {{Estimating Maximum Likelihood Parameters for Stochastic Context-Free Graph Grammars}},
  BOOKTITLE = {{The 13th Annual International Conference on Inductive Logic Programming}},
  YEAR      = {2003},
}
@Book{piaget:1952,
  AUTHOR    = {J. Piaget},
  TITLE     = {{The Origins of Intelligence in Children}},
  PUBLISHER = {International Universities Press},
  YEAR      = {1952},
}
@Book{piaget:1954,
  AUTHOR    = {J. Piaget},
  TITLE     = {{The Construction of Reality in the Child}},
  PUBLISHER = {Basic Books},
  YEAR      = {1954},
}
@Book{piaget:1963,
  AUTHOR    = {J. Piaget},
  TITLE     = {{The Origins of Intelligence in Children}},
  PUBLISHER = {W. W. Norton},
  YEAR      = {1963},
}
@InProceedings{thrun+schwartz:1995,
  AUTHOR    = {S. Thrun and A. Schwartz},
  TITLE     = {{Finding Structure in Reinforcement Learning}},
  BOOKTITLE = {{Advances in Neural Information Processing Systems}},
  YEAR      = {1995},
}
@Article{bernstein:1999,
  AUTHOR    = {D. Bernstein},
  TITLE     = {{Reusing Old Policies to Accelerate Learning on New MDPs}},
  JOURNAL   = {Technical Report UM-CS-1999-026, Dept. of CS, U. of Mass., Amherst},
  YEAR      = {1999},
}
@Book{sutton+barto:1998,
  AUTHOR    = {R. Sutton and A. Barto},
  TITLE     = {{Reinforcement Learning: An Introduction}},
  PUBLISHER = {MIT Press},
  YEAR      = {1998},
}
@Book{young:1970,
  AUTHOR    = {J. Z. Young},
  TITLE     = {{Anatomy of the Nervous System of Octopus Vulgaris}},
  PUBLISHER = {Clarendon Press},
  YEAR      = {1970},
}
@Book{hawkins+blakeslee:2004,
  AUTHOR    = {J. Hawkins and S. Blakeslee},
  TITLE     = {{On Intelligence}},
  PUBLISHER = {Times Books},
  YEAR      = {2004},
}
@InProceedings{hopcroft+wong:1974,
  AUTHOR    = {J. Hopcroft and J. Wong},
  TITLE     = {{A Linear Time Algorithm for Isomorphism of Planar Graphs}},
  BOOKTITLE = {{Proceedings of the Sixth Annual ACM Symposium on Theory of Computing}},
  PAGES     = {310-324},
  YEAR      = {1974},
}
@Article{skiena:1990,
  AUTHOR    = {S. Skiena},
  TITLE     = {{Graph Isomorphism}},
  JOURNAL   = {Implementing Discrete Mathematics: Combinatorics and Graph Theory with Mathematica},
  PUBLISHER = {Addison-Wesley},
  PAGES     = {181-187},
  YEAR      = {1990},
}
@Article{leslie+keeble:1987,
  AUTHOR    = {A. M. Leslie and S. Keeble},
  TITLE     = {{Do Six-month-old Infants Perceive Causality?}},
  JOURNAL   = {Cognition},
  PAGES     = {265-288},
  YEAR      = {1987},
}
@Article{mckay:1981,
  AUTHOR    = {B. McKay},
  TITLE     = {{Practical Graph Isomorphism}},
  JOURNAL   = {Congressus Numerantium},
  VOLUME    = {30},
  PAGES     = {45-87},
  YEAR      = {1981},
}
@Book{keller:1903,
  AUTHOR    = {H. Keller},
  TITLE     = {{The Story of My Life}},
  YEAR      = {1903},
}
@Book{hoppner+klawonn+kruse+runkler:1999,
  AUTHOR    = {F. Hoppner and F. Klawonn and R. Kruse and T. Runkler},
  TITLE     = {{Fuzzy Cluster Analysis}},
  PUBLISHER = {Wiley},
  YEAR      = {1999},
}
@InProceedings{gonzalez+holder+cook:2002,
  AUTHOR    = {J. A. Gonzalez and L. B. Holder and D. J. Cook},
  TITLE     = {{Graph Based Relational Concept Learning}},
  BOOKTITLE = {{Proceedings of the International Conference on Machine Learning}},
  YEAR      = {2002},
  ADDRESS   = {}
}
@Article{gentner:1983,
  AUTHOR    = {D. Gentner},
  TITLE     = {{Structure-Mapping: A Theoretical Framework for Analogy}},
  JOURNAL   = {Cognitive Science},
  YEAR      = {1983},
  VOLUME    = {7},
  PAGES     = {155-170},
}
@Article{dietrich:2000,
  AUTHOR    = {E. Dietrich},
  TITLE     = {{Analogy and Conceptual Change, or You Can't Step into the Same Mind Twice}},
  JOURNAL   = {Cognitive Dynamics: Conceptual Change in Humans and Machines},
  PAGES     = {265-294},
  YEAR      = {2000},
}
@Article{hummel+holyoak:2006,
  AUTHOR    = {J. E. Hummel and K. J. Holyoak},
  TITLE     = {{A Symbolic-Connectionist Theory of Relational Inference and Generalization}},
  JOURNAL   = {Psychological Review},
  YEAR      = {2006},
}
@InProceedings{dejong:1999,
  AUTHOR    = {E. De Jong},
  TITLE     = {{Autonomous Concept Formation}},
  BOOKTITLE = {{Proceedings of the International Joint Conference on Artificial Intelligence}},
  YEAR      = {1999},
}
@Article{odonoghue:2005,
  AUTHOR    = {D. O'Donoghue},
  TITLE     = {{Finding Novel Analogies}},
  JOURNAL   = {PhD Thesis, University College Dublin},
  YEAR      = {2005},
}
@Article{oates:2000,
  AUTHOR    = {Tim Oates},
  TITLE     = {{Grounding Knowledge in Sensors: Unsupervised Learning for Language and Planning}},
  JOURNAL   = {PhD Thesis, University of Massachusetts Amherst},
  YEAR      = {2000},
}
@InProceedings{holder+cook+djoko:1994,
  AUTHOR    = {L. Holder and D. Cook and S. Djoko},
  TITLE     = {{Substructure Discovery in the SUBDUE System}},
  BOOKTITLE = {{Workshop on Knowledge Discovery in Databases}},
  YEAR      = {1994},
  ADDRESS   = {}
}
@InProceedings{marshall+hofstadter:1996,
  AUTHOR    = {J. B. D. Marshall and D. R. Hofstadter},
  TITLE     = {{Beyond Copycat: Incorporating Self-Watching into a Computer Model of High-Level Perception and Analogy-Making}},
  BOOKTITLE = {{Online Proceedings of the 1996 Midwest Artificial Intelligence and Cognitive Science Conference}},
  YEAR      = {1996},
}
@Article{forbus:2001,
  AUTHOR    = {K. Forbus},
  TITLE     = {{Exploring Analogy in the Large}},
  JOURNAL   = {The Analogical Mind: Perspectives from Cognitive Science},
  YEAR      = {2001},
  PUBLISHER = {The MIT Press/Bradford Books},
}
@Article{falkenhainer+forbus+gentner:1989,
  AUTHOR    = {B. Falkenhainer and K. Forbus and D. Gentner},
  TITLE     = {{The Structure Mapping Engine: Algorithm and Examples}},
  JOURNAL   = {Artificial Intelligence},
  YEAR      = {1989},
}
@Article{hofstadter:2001,
  AUTHOR    = {D. R. Hofstadter},
  TITLE     = {{Analogy as the Core of Cognition}},
  JOURNAL   = {The Analogical Mind: Perspectives from Cognitive Science},
  PAGES     = {499-538},
  YEAR      = {2001},
  PUBLISHER = {The MIT Press/Bradford Books},
}
@Article{hofstadter:1984,
  AUTHOR = {D. R. Hofstadter},
  TITLE = {{The Copycat Project: An Experiment in Nondeterminism and Creative Analogies}},
  JOURNAL = {Massachusetts Institute of Technology},
  VOLUME = {755},
  YEAR = {1984},
}
@Article{nevillmanning97compression,
  AUTHOR    = {C. G. Nevill-Manning and I. H. Witten},
  TITLE     = {{Compression and Explanation Using Hierarchical Grammars}},
  JOURNAL   = {The Computer Journal},
  VOLUME    = {40},
  NUMBER    = {2/3},
  PAGES     = {103},
  YEAR      = {1997},
}
@Article{thompson+langley:1991,
  AUTHOR    = {K. Thompson and P. Langley},
  TITLE     = {{Concept formation in structured domains}},
  JOURNAL   = {Concept Formation: Knowledge and Experience in Unsupervised Learning (D. H. Fisher and M. Pazzani, editors)},
  YEAR      = {1991},
  PAGES     = {Chapter 5},
  PUBLISHER = {Morgan Kaufmann Publishers},
}
@Article{cohen:1998,
  AUTHOR    = {P. Cohen},
  TITLE     = {{Growing Ontologies}},
  JOURNAL   = {Technical Report 98-20, The University of Massachusetts, Amherst},
  YEAR      = {1998},
}
@InProceedings{rosenstein+cohen:1999,
  AUTHOR    = {M. Rosenstein and P. Cohen},
  TITLE     = {{Continuous Categories for a Mobile Robot}},
  BOOKTITLE = {{proceedings of the 16th National Conference on Artificial Intelligence}},
  YEAR      = {1999},
}
@Article{iba+langley:2001,
  AUTHOR    = {W. Iba and P. Langley},
  TITLE     = {{Unsupervised Learning of Probabilistic Concept Hierarchies}},
  JOURNAL   = {Lecture Notes in Computer Science},
  VOLUME    = {2049},
  YEAR      = {2001},
  PAGES     = {39},
}
@Article{nagel+schreckenberg:1995,
  AUTHOR    = {K. Nagel and M. Schreckenberg},
  TITLE     = {{Traffic Jam Dynamics in Stochastic Cellular Automata}},
  JOURNAL   = {Los Alamos National Laboratories technical report},
  YEAR      = {1995},
}
@InProceedings{cohen+heeringa+adams:2002,
  TYPE      = {peer-reviewed-conference},
  AUTHOR    = {Paul R. Cohen and Brent Heeringa and Niall Adams},
  TITLE     = {{An Unsupervised Algorithm for Segmenting Categorical Time Series into Episodes}},
  BOOKTITLE = {{Proceedings of the 2002 IEEE International Conference on Data Mining (ICDM 2002)}},
  PAGES     = {99-106},
  YEAR      = {2002},
}
@Article{wolff:2003,
  AUTHOR    = {J. G. Wolff},
  TITLE     = {{Information Compression by Multiple Alignment, Unification and Search as a Unifying Principle in Computing and Cognition}},
  JOURNAL   = {Artif. Intell. Rev.},
  VOLUME    = {19},
  NUMBER    = {3},
  YEAR      = {2003},
  ISSN      = {0269-2821},
  PAGES     = {193-230},
  PUBLISHER = {Kluwer Academic Publishers},
}
@Misc{Blake+Merz:1998,
  AUTHOR      = {C.L. Blake and C.J. Merz},
  YEAR        = {1998},
  TITLE       = {{UCI Repository of Machine Learning Databases}},
  INSTITUTION = {University of California, Irvine, Dept. of Information and Computer Sciences},
}
@InProceedings{gruber:1993,
  AUTHOR    = {T. R. Gruber},
  TITLE     = {{Towards Principles for the Design of Ontologies Used for Knowledge Sharing}},
  BOOKTITLE = {{Formal Ontology in Conceptual Analysis and Knowledge Representation}},
  PUBLISHER = {Kluwer Academic Publishers},
  ADDRESS   = {Deventer, The Netherlands},
  EDITOR    = {N. Guarino and R. Poli},
  YEAR      = {1993},
}
@Article{olson:1995,
  AUTHOR    = {Clark F. Olson},
  TITLE     = {{Parallel algorithms for hierarchical clustering}},
  JOURNAL   = {Parallel Computing},
  VOLUME    = {21},
  NUMBER    = {8},
  PAGES     = {1313-1325},
  YEAR      = {1995},
}
@Misc{fasulo:1999,
  AUTHOR    = {D. Fasulo},
  TITLE     = {{An Analysis of Recent Work on Clustering Algorithms}},
  YEAR      = {1999},
}
@Book{ganter+wille:1999,
  AUTHOR    = {B. Ganter and R. Wille},
  TITLE     = {{Formal Concept Analysis: Mathematical Foundations}},
  ADDRESS   = {New York},
  PUBLISHER = {Springer-Verlag},
  YEAR      = {1999},
}
@Article{pierce+kuipers:1997,
  AUTHOR    = {D. Pierce and B. Kuipers},
  TITLE     = {{Map learning with Uninterpreted Sensors and Effectors}},
  JOURNAL   = {Artificial Intelligence},
  YEAR      = {1997},
  VOLUME    = {92},
  PAGES     = {169-229},
  RATING    = {D},
  KEYWORDS  = {artificial intelligence, learning},
}
@InProceedings{zucker+bredeche+saitta:2002,
  AUTHOR    = {J.-D. Zucker and N. Bredeche and L. Saitta},
  TITLE     = {{Abstracting Visual Percepts to Learn Concepts}},
  BOOKTITLE = {{5th International Symposium on Abstraction, Reformulation and Approximation (SARA 2002)}},
  YEAR      = {2002},
  PAGES     = {256-273},
  EDITOR    = {Sven Koenig and Robert Holte},
  VOLUME    = {2371},
  SERIES    = {Lecture Notes in Artificial Intelligence},
  PUBLISHER = {Springer Verlag},
}
@InProceedings{cole:2001,
  AUTHOR    = {R. Cole},
  TITLE     = {{Automated layout of concept lattices using layered diagrams and additive diagrams}},
  BOOKTITLE = {{ACSC '01: Proceedings of the 24th Australasian conference on Computer science}},
  YEAR      = {2001},
  ISBN      = {0-7695-0963-0},
  PAGES     = {47-53},
  LOCATION  = {Gold Coast, Queensland, Australia},
  PUBLISHER = {IEEE Computer Society},
}
@Book{ehrig+engels+kreowski+rozenberg:1999,
  EDITOR    = {H. Ehrig and G. Engels and H.J. Kreowski and G. Rozenberg},
  PUBLISHER = {World Scientific Publishing Co.},
  TITLE     = {{Handbook of Graph Grammars and Computing by Graph Transformation, Volume 2: Applications, Languages and Tools}},
  YEAR      = {1999},
}
@Article{boatman+freeman+vining+pulsifer+miglioretti+minahan+carson+brandt+mckhann:1999,
  AUTHOR    = {D. Boatman and J. Freeman and E. Vining and M. Pulsifer and D. Miglioretti and R. Minahan and B. Carson and J. Brandt and G. McKhann},
  TITLE     = {{Language Recovery After Left Hemispherectomy in Children with Late-onset Seizures}},
  JOURNAL   = {Annals of Neurology},
  VOLUME    = {46 (4)},
  PAGES     = {579-86},
  YEAR      = {1999},
}
@Book{newell+simon:1972,
  AUTHOR    = {A. Newell and H. A. Simon},
  PUBLISHER = {Prentice Hall},
  TITLE     = {{Human Problem Solving}},
  YEAR      = {1972},
}
@Book{babbage:1864,
  AUTHOR    = {C. Babbage},
  PUBLISHER = {Longman, Green, Longman, Roberts, and Green},
  ADDRESS   = {London},
  TITLE     = {{Passages from the Life of a Philosopher}},
  YEAR      = {1864},
}
@Book{stafford+webb:2004,
  AUTHOR = {T. Stafford and M. Webb},
  PUBLISHER = {O'Reilly Media, Inc.},
  TITLE = {{Mind Hacks: Tips \& Tools for Using Your Brain}},
  YEAR = {2004},
}
@Article{cassimatis:2006,
  AUTHOR = {N. L. Cassimatis},
  TITLE = {{A Cognitive Substrate for Achieving Human-Level Intelligence}},
  JOURNAL = {AI Magazine},
  VOLUME = {27},
  NUMBER = {2},
  YEAR = {2006},
  ISSN = {0738-4602},
  PAGES = {45--56},
  PUBLISHER = {American Association for Artificial Intelligence},
  ADDRESS = {Menlo Park, CA, USA},
}
@InProceedings{levy+gayler:2008,
  AUTHOR    = {S. D. Levy and R. Gayler},
  TITLE     = {{Vector Symbolic Architectures: A New Building Material for Artificial General Intelligence}},
  BOOKTITLE = {{Proceedings of The First Conference on Artificial General Intelligence}},
  YEAR      = {2008},
}
@InProceedings{munos+moore:1999,
  AUTHOR = {R. Munos and A. W. Moore},
  TITLE = {{Variable Resolution Discretization for High-Accuracy Solutions of Optimal Control Problems}},
  BOOKTITLE = {{Proceedings of the International Joint Conference on Artificial Intelligence}},
  YEAR = {1999},
}
@Book{watson:1968,
  AUTHOR = {J. D. Watson},
  PUBLISHER = {Simon and Schuster},
  TITLE = {{The Double Helix: A Personal Account of the Discovery of the Structure of DNA}},
  YEAR = {1968},
}
@Book{schopenhauer:1844,
  AUTHOR = {A. Schopenhauer},
  TITLE = {{Die Welt als Wille und Vorstellung, Bde. I \& II (The World as Will and Representation, Vols. I \& II)}},
  YEAR = {1844},
}
@Book{maclean:1990,
  AUTHOR = {P. D. MacLean},
  PUBLISHER = {Plenum Press},
  ISBN      = {0-306-43168-8},
  ADDRESS   = {New York},
  TITLE = {{The Triune Brain in Evolution: Role in Paleocerebral Functions}},
  YEAR = {1990},
}
@Book{damasio:2000,
  AUTHOR = {A. R. Damasio},
  PUBLISHER = {Vintage},
  ISBN      = {0099288761},
  TITLE = {{The Feeling of What Happens: Body, Emotion and the Making of Consciousness}},
  YEAR = {2000},
}
@Book{minsky:1988,
  AUTHOR = {M. Minsky},
  PUBLISHER = {Simon \& Schuster},
  TITLE = {{Society of Mind}},
  YEAR = {1988},
}
@Book{hofstadter:1979,
  AUTHOR = {D. R. Hofstadter},
  PUBLISHER = {Basic Books},
  TITLE = {{G\"odel, Escher, Bach: an Eternal Golden Braid}},
  YEAR = {1979},
}
@Book{stock:1987,
  AUTHOR = {G. Stock},
  PUBLISHER = {Workman Publishing Company},
  TITLE = {{The Book of Questions}},
  YEAR = {1987},
}
@Book{ditfurth:1981,
  AUTHOR = {H. v. Ditfurth},
  PUBLISHER = {Hoffman und Campe},
  TITLE = {{Wir sind nicht nur von dieser Welt}},
  YEAR = {1981},
}
@Article{riesenhuber+poggio:1999,
  AUTHOR = {M. Riesenhuber and T. Poggio},
  TITLE = {{Hierarchical Models of Object Recognition in Cortex}},
  JOURNAL = {{Nature Neuroscience}},
  VOLUME = {2},
  NUMBER = {11},
  YEAR = {1999},
  ISSN = {1097-6256},
  PAGES = {1019--1025},
  ADDRESS = {Department of Brain and Cognitive Sciences, Center for Biological and Computational Learning and Artificial Intelligence Laboratory, Massachusetts Institute of Technology, Cambridge, Massachusetts 02142, USA.},
}
@Book{garey+johnson:1990,
  AUTHOR = {Garey, M. R. and Johnson, D. S.},
  PUBLISHER = {W. H. Freeman \& Co.},
  ADDRESS = {New York, NY, USA},
  TITLE = {{Computers and Intractability; A Guide to the Theory of NP-Completeness}},
  YEAR = {1990},
}
@incollection{karp:1972,
    author = {Karp, R. M.},
    booktitle = {{Complexity of Computer Computations}},
    citeulike-article-id = {1923170},
    editor = {Miller, R. E. and Thatcher, J. W.},
    keywords = {bibtex-import, file-import-09-01-22},
    pages = {85--103},
    posted-at = {2007-11-15 16:43:57},
    priority = {2},
    publisher = {Plenum Press},
    title = {{Reducibility Among Combinatorial Problems}},
    year = {1972}
}
@Article{cooper:1990,
 AUTHOR = {Cooper, G. F.},
 TITLE = {{The Computational Complexity of Probabilistic Inference using Bayesian Belief Networks}},
 JOURNAL = {Artificial Intelligence},
 VOLUME = {42},
 NUMBER = {2-3},
 YEAR = {1990},
 ISSN = {0004-3702},
 PAGES = {393--405},
 DOI = {http://dx.doi.org/10.1016/0004-3702(90)90060-D},
 PUBLISHER = {Elsevier Science Publishers Ltd.},
 ADDRESS = {Essex, UK},
}
@Book{wolfram:2002,
  AUTHOR = {Wolfram, S},
  PUBLISHER = {Wolfram Media},
  ADDRESS = {New York, NY, USA},
  TITLE = {{A New Kind of Science}},
  YEAR = {2002},
}
@Article{nagel:1974,
 AUTHOR = {T. Nagel},
 TITLE = {{What is it Like to Be a Bat?}},
 JOURNAL = {The Philosophical Review},
 VOLUME = {83},
 NUMBER = {4},
 YEAR = {1974},
 PAGES = {435-450},
}
@InProceedings{plate:1991,
 author = {T. Plate},
 title = {{Holographic Reduced Representations: Convolution Algebra for Compositional Distributed Representations}},
 booktitle = {{International Joint Conference on Artificial Intelligence}},
 year = {1991},
 publisher = {Morgan Kaufmann}
}
@Book{nietzsche:1885,
  AUTHOR = {F. Nietzsche},
  PUBLISHER = {Walter de Gruyter \& Co.},
  ADDRESS = {Berlin},
  TITLE = {{Also Sprach Zarathustra: Ein Buch f\"ur Alle und Keinen}},
  YEAR = {1885},
}
@Book{boorstin:1994,
  AUTHOR = {D. Boorstin},
  PUBLISHER = {Random House},
  ADDRESS = {New York},
  TITLE = {{Cleopatra's Nose: Essays on the Unexpected}},
  YEAR = {1994},
}
@Book{bortoft:1996,
  AUTHOR = {H. Bortoft},
  PUBLISHER = {Lindisfarne Books},
  ADDRESS = {Great Barrington, Massachusetts},
  TITLE = {{The Wholeness Of Nature: Goethe's Way toward a Science of Conscious Participation in Nature}},
  YEAR = {1996},
}
@Book{quine:1995,
  AUTHOR = {W. V. O. Quine},
  PUBLISHER = {Harvard University Press},
  ADDRESS = {Cambridge, Massachusetts},
  TITLE = {{From Stimulus to Science}},
  YEAR = {1995},
}
@article{gopnik:1998,
 AUTHOR = {A. Gopnik},
 TITLE = {{Explanation as Orgasm}},
 JOURNAL = {Minds Machines},
 VOLUME = {8},
 NUMBER = {1},
 YEAR = {1998},
 ISSN = {0924-6495},
 PAGES = {101--118},
 PUBLISHER = {Kluwer Academic Publishers},
 ADDRESS = {Hingham, Massachusetts},
}
@Book{gopnik+meltzoff:1997,
  AUTHOR = {A. Gopnik and A. N. Meltzoff},
  PUBLISHER = {Bradford Books},
  ADDRESS = {Cambridge, Massachusetts},
  TITLE = {{Words, Thoughts, and Theories}},
  YEAR = {1997},
}
@Book{gladwell:2000,
  AUTHOR = {M. Gladwell},
  PUBLISHER = {Little, Brown},
  ADDRESS = {New York},
  TITLE = {{The Tipping Point: How Little Things Can Make a Big Difference}},
  YEAR = {2000},
}
@Book{gladwell:2005,
  AUTHOR = {M. Gladwell},
  PUBLISHER = {Little, Brown},
  ADDRESS = {New York},
  TITLE = {{Blink: The Power of Thinking Without Thinking}},
  YEAR = {2005},
}
@Book{surowiecki:2004,
  AUTHOR = {J. Surowiecki},
  PUBLISHER = {Doubleday},
  ADDRESS = {New York},
  TITLE = {{The Wisdom of Crowds: Why the Many Are Smarter Than the Few and How Collective Wisdom Shapes Business, Economies, Societies and Nations}},
  YEAR = {2004},
}
@Book{westervelt+grizzle+chevallereau+choi+morris:2007,
  AUTHOR = {E. R. Westervelt and J. W. Grizzle and C. Chevallereau and J. H. Choi and B. Morris},
  PUBLISHER = {Taylor \& Francis/CRC},
  ADDRESS = {New York},
  TITLE = {{Feedback Control of Dynamic Bipedal Robot Locomotion}},
  YEAR = {2007},
}
@Book{hume:1740,
  AUTHOR    = {D. Hume},
  TITLE     = {{A Treatise of Human Nature}},
  YEAR      = {1740},
}
@Book{jevons:1866,
  AUTHOR = {W. S. Jevons},
  PUBLISHER = {Macmillan \& Co.},
  ADDRESS = {London},
  TITLE = {{The Coal Question}},
  YEAR = {1866},
}
@article{good:1965,
 AUTHOR = {I. J. Good},
 TITLE = {{Speculations Concerning the First Ultraintelligent Machine}},
 JOURNAL = {Advances in Computers},
 VOLUME = {6},
 YEAR = {1965},
}

@inproceedings{DBLP:conf/icml/KiraR92,
  author    = {Kenji Kira and
               Larry A. Rendell},
  title     = {A Practical Approach to Feature Selection},
  booktitle = {ML},
  year      = {1992},
  pages     = {249-256},
  crossref  = {DBLP:conf/icml/1992},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}


@article{shanker+richtel:2011,
 AUTHOR = {T. Shanker and M. Richtel},
 TITLE = {{In new military, data overload can be deadly}},
 JOURNAL = {New York Times},
 VOLUME = {January 15},
 YEAR = {2011},
}

@book{zacharias2008behavioral,
  title={Behavioral modeling and simulation: from individuals to societies},
  author={Zacharias, G. and MacMillan, J. and Van Hemel, S.B.},
  year={2008},
  publisher={National Academy Press}
}

@article{salvucci2006modeling,
  title={Modeling driver behavior in a cognitive architecture},
  author={Salvucci, D.D.},
  journal={Human Factors: The Journal of the Human Factors and Ergonomics Society},
  volume={48},
  number={2},
  pages={362--380},
  year={2006},
  publisher={SAGE Publications}
}

@article{liao2012act,
  title={An ACT-R model of credibility judgment of micro-blogging web pages},
  author={Liao, Q.V. and Pirolli, P. and Fu, W.T.},
  journal={ICCM 2012 Proceedings},
  pages={103},
  year={2012},
  publisher={Univerlagtuberlin}
}

@inproceedings{DBLP:conf/eccv/LeCun12,
  author    = {Yann LeCun},
  title     = {Learning Invariant Feature Hierarchies},
  booktitle = {ECCV Workshops (1)},
  year      = {2012},
  pages     = {496-505},
  ee        = {http://dx.doi.org/10.1007/978-3-642-33863-2_51},
  crossref  = {DBLP:conf/eccv/2012w1},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}
@proceedings{DBLP:conf/eccv/2012w1,
  editor    = {Andrea Fusiello and
               Vittorio Murino and
               Rita Cucchiara},
  title     = {Computer Vision - ECCV 2012. Workshops and Demonstrations
               - Florence, Italy, October 7-13, 2012, Proceedings, Part
               I},
  booktitle = {ECCV Workshops (1)},
  publisher = {Springer},
  series    = {Lecture Notes in Computer Science},
  volume    = {7583},
  year      = {2012},
  isbn      = {978-3-642-33862-5},
  ee        = {http://dx.doi.org/10.1007/978-3-642-33863-2},
  bibsource = {DBLP, http://dblp.uni-trier.de}
}

@article{wharton1996remote,
  title={{Remote Analogical Reminding}},
  author={Wharton, C.M. and Holyoak, K.J. and Lange, T.E.},
  journal={Memory \& Cognition},
  volume={24},
  number={5},
  pages={629--643},
  year={1996},
  publisher={Springer}
}

@article{mountcastle1978organizing,
  title={{An Organizing Principle for Cerebral Function: The Unit Model and the Distributed System}},
  author={Mountcastle, V.},
  journal={The Mindful Brain},
  year={1978},
  pages={7--50},
  publisher={MIT press}
}

@article{mountcastle1978organizingShort,
  title={{An Organizing Principle for Cerebral Function: The Unit Model and the Distributed System}},
  author={Mountcastle, V.},
  year={1978},
  publisher={MIT press}
}

@inproceedings{si2011unsupervised,
  title={{Unsupervised Learning of Stochastic AND-OR Templates for Object Modeling}},
  author={Si, Z. and Zhu, S.C.},
  booktitle={{IEEE Int. Conf. on Computer Vision Workshops}},
  pages={648--655},
  year={2011},
  organization={IEEE},
  address={}
}

@inproceedings{gayler2009distributed,
  title={{A Distributed Basis for Analogical Mapping}},
  author={Gayler, R.W. and Levy, S.D.},
  booktitle={{New Frontiers in Analogy Research; Proc. of 2nd Intern. Analogy Conf.}},
  year={2009},
  address={}
}

@inproceedings{clement1987generation,
  title={{Generation of Spontaneous Analogies by Students Solving Science Problems}},
  author={Clement, J.},
  booktitle={{Thinking Across Cultures}},
  year={1987},
  pages={303-308},
  address={}
}

@article{clement1988observed,
  title={{Observed methods for generating analogies in scientific problem solving}},
  author={Clement, J.},
  journal={Cognitive Science},
  volume={12},
  number={4},
  pages={563--586},
  year={1988},
  publisher={Elsevier}
}

@article{roth2005evolution,
  title={{Evolution of the Brain and Intelligence}},
  author={Roth, Gerhard and Dicke, Ursula},
  journal={Trends in Cognitive Sciences},
  volume={9},
  number={5},
  pages={250--257},
  year={2005},
  publisher={Elsevier}
}

@article{rakic2009evolution,
  title={{Evolution of the Neocortex: A Perspective from Developmental Biology}},
  author={Rakic, Pasko},
  journal={Nature Reviews Neuroscience},
  volume={10},
  number={10},
  pages={724--735},
  year={2009},
  publisher={Nature Publishing Group}
}

@article{borner2001efficient,
  title={Efficient case-based structure generation for design support},
  author={B{\"o}rner, Katy},
  journal={Artificial Intelligence Review},
  volume={16},
  number={2},
  pages={87--118},
  year={2001},
  publisher={Springer}
}

@article{albus1971theory,
  title={A theory of cerebellar function},
  author={Albus, James S},
  journal={Mathematical Biosciences},
  volume={10},
  number={1},
  pages={25--61},
  year={1971},
  publisher={Elsevier}
}

